Tight Cutoffs for Guarded Protocols with Fairness

Guarded protocols were introduced in a seminal paper by Emerson and Kahlon (2000), and describe systems of processes whose transitions are enabled or disabled depending on the existence of other processes in certain local states. We study parameterized model checking and synthesis of guarded protocols, both aiming at formal correctness arguments for systems with any number of processes. Cutoff results reduce reasoning about systems with an arbitrary number of processes to systems of a determined, fixed size. Our work stems from the observation that existing cutoff results for guarded protocols i) are restricted to closed systems, and ii) are of limited use for liveness properties because reductions do not preserve fairness. We close these gaps and obtain new cutoff results for open systems with liveness properties under fairness assumptions. Furthermore, we obtain cutoffs for the detection of global and local deadlocks, which are of paramount importance in synthesis. Finally, we prove tightness or asymptotic tightness for the new cutoffs.

==> ams_proof.tex <==
\DeclareRobustCommand{\qed}{%
  \ifmmode \mathqed
  \else
    \leavevmode\unskip\penalty9999 \hbox{}\nobreak\hfill
    \quad\hbox{\qedsymbol}%
  \fi
}
\let\QED@stack\@empty
\let\qed@elt\relax
\newcommand{\pushQED}[1]{%
  \toks@{\qed@elt{#1}}\@temptokena\expandafter{\QED@stack}%
  \xdef\QED@stack{\the\toks@\the\@temptokena}%
}
\newcommand{\popQED}{%
  \begingroup\let\qed@elt\popQED@elt \QED@stack\relax\relax\endgroup
}
\def\popQED@elt#1#2\relax{#1\gdef\QED@stack{#2}}
\newcommand{\qedhere}{%
  \begingroup \let\mathqed\math@qedhere
    \let\qed@elt\setQED@elt \QED@stack\relax\relax \endgroup
}
\newif\ifmeasuring@
\newif\iffirstchoice@ \firstchoice@true
\def\setQED@elt#1#2\relax{%
  \ifmeasuring@
  \else \iffirstchoice@ \gdef\QED@stack{\qed@elt{}#2}\fi
  \fi
  #1%
}
\def\qed@warning{%
  \PackageWarning{amsthm}{The \@nx\qedhere command may not work
    correctly here}%
}
\newcommand{\mathqed}{\quad\hbox{\qedsymbol}}
\def\linebox@qed{\hfil\hbox{\qedsymbol}\hfilneg}
\@ifpackageloaded{amsmath}{%
  \def\math@qedhere{%
    \@ifundefined{\@currenvir @qed}{%
      \qed@warning\quad\hbox{\qedsymbol}%
    }{%
      \@xp\aftergroup\csname\@currenvir @qed\endcsname
    }%
  }
  \def\displaymath@qed{%
    \relax
    \ifmmode
      \ifinner \aftergroup\linebox@qed
      \else
        \eqno
        \let\eqno\relax \let\leqno\relax \let\veqno\relax
        \hbox{\qedsymbol}%
      \fi
    \else
       \aftergroup\linebox@qed
    \fi
  }
  \@xp\let\csname equation*@qed\endcsname\displaymath@qed
  \def\equation@qed{%
    \iftagsleft@
      \hbox{\phantom{\quad\qedsymbol}}%
      \gdef\alt@tag{%
        \rlap{\hbox to\displaywidth{\hfil\qedsymbol}}%
        \global\let\alt@tag\@empty
      }%
    \else
      \gdef\alt@tag{%
        \global\let\alt@tag\@empty
        \vtop{\ialign{\hfil####\cr
                \tagform@\theequation\cr
                \qedsymbol\cr}}%
        \setbox\z@
      }%
    \fi
  }
  \def\qed@tag{%
    \global\tag@true \nonumber
    &\omit\setboxz@h {\strut@ \qedsymbol}\tagsleft@false
    \place@tag@gather
    \kern-\tabskip
    \ifst@rred \else \global\@eqnswtrue \fi \global\advance\row@\@ne \cr
  }
  \def\split@qed{%
    \def\endsplit{\crcr\egroup \egroup \ctagsplit@false \rendsplit@
      \aftergroup\align@qed
    }%
  }
  \def\align@qed{%
    \ifmeasuring@ \tag*{\qedsymbol}%
    \else \let\math@cr@@@\qed@tag
    \fi
  }
  \@xp\let\csname align*@qed\endcsname\align@qed
  \@xp\let\csname gather*@qed\endcsname\align@qed
%% Needs some patching up for amsmath 1.2
}{% end of amsmath branch, start plain LaTeX branch
  \def\math@qedhere{%
    \@ifundefined{\@currenvir @qed}{%
      \qed@warning \aftergroup\displaymath@qed
    }{%
      \@xp\aftergroup\csname\@currenvir @qed\endcsname
    }%
  }
  \def\displaymath@qed{%
    \relax
    \ifmmode
      \ifinner \aftergroup\aftergroup\aftergroup\linebox@qed
      \else
        \eqno \def\@badmath{$$}%
        \let\eqno\relax \let\leqno\relax \let\veqno\relax
        \hbox{\qedsymbol}%
      \fi
    \else
       \aftergroup\linebox@qed
    \fi
  }
  \@ifundefined{ver@leqno.clo}{%
    \def\equation@qed{\displaymath@qed \quad}%
  }{%
    \def\equation@qed{\displaymath@qed}%
  }
    \def\@tempa#1$#2#3\@nil#4{%
        \def#4{#1$#2\def\@currenvir{displaymath}#3}%
    }%
    \expandafter\ifx\csname[ \endcsname\relax
        \expandafter\@tempa\[\@nil\[%
    \else
        \expandafter\expandafter\expandafter\@tempa\csname[
        \expandafter\endcsname\expandafter\@nil
        \csname[ \endcsname
    \fi
}
\@ifpackageloaded{amstex}{%
  \def\@tempa{TT}%
}{%
  \@ifpackageloaded{amsmath}{%
    \def\@tempb#1 v#2.#3\@nil{#2}%
    \ifnum\@xp\@xp\@xp\@tempb\csname ver@amsmath.sty\endcsname v0.0\@nil
       <\tw@
      \def\@tempa{TT}%
    \else
      \def\@tempa{TF}%
    \fi
  }{%
    \def\@tempa{TF}
  }%
}
\if\@tempa
  \renewcommand{\math@qedhere}{\quad\hbox{\qedsymbol}}%
\fi
\newcommand{\openbox}{\leavevmode
  \hbox to.77778em{%
  \hfil\vrule
  \vbox to.675em{\hrule width.6em\vfil\hrule}%
  \vrule\hfil}}
\DeclareRobustCommand{\textsquare}{%
  \begingroup \usefont{U}{msa}{m}{n}\thr@@\endgroup
}
\providecommand{\qedsymbol}{\openbox}
\newenvironment{proof}[1][\proofname]{\par
  \pushQED{\qed}%
  \normalfont \topsep6\p@\@plus6\p@\relax
  \trivlist
  \item[\hskip\labelsep
        \itshape
    #1\@addpunct{.}]\ignorespaces
}{%
  \popQED\endtrivlist\@endpefalse
}
\providecommand{\proofname}{Proof}

==> conversion.tex <==
\subsection{Translation Between Open and Closed Systems}
\sj{short description of approach and drawbacks (translation blows up state-space (and thus, cutoffs); does not include any notion of fairness, i.e., only suitable for safety verification)}
In general, the cut-off results for guarded systems can only be used for synthesizing closed systems. However, we provide an algorithm that allows to convert any open system into an equivalent closed system and vice versa. In the corresponding closed system, the environment's behaviour is modelled by non-determinism regarding the transition relations. Applying the inverse conversion to a synthesized closed system yields an open system. To this end, we iteratively convert each open LTS $\mathcal{T}_i = (T_i, t_i, \delta_i, o_i)$ into an equivalent closed LTS in two steps. In the first step, we construct an input-preserving LTS $\mathcal{T}_i^{\text{ip}} = (T_i \times \mathcal{P}(I_i), t_i \times {\_}, \delta_i, o_i)$, such that for each transition $(t, i', t')$ of the given open LTS and each $(t,i) \in T_i \times \mathcal{P}(I_i)$ corresponding to an original state $t \in T_i$, there exists a corresponding transition $((t,i), i', (t',i))$ in the new system. Thus, the last read input values are stored in the current state. In the second step, we remove the input labels from all transitions defined by the transition relation $\delta$. The resulting system does not depend on environment inputs and thus is a closed system. However, each local state still contains information about input values. Whereas these input values are provided by the environment in the open system, the corresponding closed system decides about the input values by selecting a certain transition, and thus a particular set of input values provided by the successor state.

This conversion algorithm allows us to directly use the cut-off results for closed systems. However, a major drawback is the worst-case exponential state blow-up, which is caused by the conversion of the open system to the input-preserving LTS. As a result, there is also an exponential cut-off increase, because the cut-offs are proportional to the state size (i.e., bound). A further issue is the absence of fairness constraints, which allows to synthesize systems that only satisfy specifications that contain safety properties only.


==> encoding.tex <==
\section{Bounded Template Synthesis}

The cutoffs in Section~\ref{sec:cutoffs} allow us to %solve the
reduce parameterized synthesis to template synthesis for a fixed number of processes. 
%For distributed architectures that do not fall into decidable classes,
Finkbeiner and Schewe have introduced \emph{bounded
  synthesis}~\cite{FinkbeinerS13}, a semi-decision procedure
that converts a (generally undecidable)
distributed synthesis problem into a sequence of decidable synthesis problems,
by bounding the size of the implementation. In the following, we
introduce the main ideas of the original approach and describe how to adapt 
the procedure for template synthesis of guarded protocols.



\subsection{Bounded Synthesis Method}
\label{sec:bounded_synthesis}
Bounded synthesis consists of three main steps:

\subsubsection*{Step 1: Automata translation}
 The
  LTL specification $\spec$, including fairness assumptions
like fair scheduling, is translated (according to \cite{KupfermanV05}) into a universal co-B\"uchi automaton $\mU$ that
accepts an LTS if and only if the LTS satisfies $\spec$.

\subsubsection*{Step 2: SMT Encoding} Existence of an LTS of size $b$ 
that satisfies $\spec$ is encoded into a set of SMT constraints. 
States are represented by natural numbers in %the range 
$S=\{1, \ldots, b\}$, state labels as free functions of type $S \impl \bbB$, 
and the global transition function as a free function of type $S \times 
\bbB^{E} \impl  S$. Transitions of individual processes are defined 
%indirectly 
by introducing projections $d_i: S \impl S$, mapping global to 
local states. Additional constraints ensure that local transitions only 
depend on local information. 

%of process $i$ only depend on inputs in $I_i$, we add a constraint
%\[ \bigwedge_{i \in P^-} ~ \bigwedge_{t,t' \in T} ~ \bigwedge_{I,I' \in \mathcal{P}(O_{env})}~ d_i(t) = d_i(t') \land I \cap I_i = I'
%\cap I_i \impl d_i(\delta(t,I)) = d_i(\delta(t',I')).\]

To obtain an interpretation of these symbols that satisfies the
specification $\spec$, additional annotations of states are
introduced. This includes labels $\lambda^\bbB_q: S \impl \bbB$
and free functions $\lambda^\#_q: S \impl \bbR$, defined
such that (i) $\lambda^\bbB_q(s)$ is true if and only if $(q,t) \in Q \times S$
is reachable in a run of $\mU$ on the LTS\footnote{That is, there is a
  run of $\mU$ on the LTS such that at some point $q$ is among the
  states of $\mU$ when it reads (the label of) state $s$.},
and (ii) valuations of the 
$\lambda^\#_q$ must be increasing along paths of $\mU$, and strictly
increasing for transitions that enter a rejecting state of
$\mU$. Together, this ensures that an LTS satisfying these constraints
cannot have runs which enter rejecting states infinitely often (and
thus would be rejected by $\mU$).

%% To obtain an interpretation of these symbols that satisfies the specification
%% $\spec$, additional annotations of states are introduced. This includes labels
%% $\lambda^\bbB_q: \bbN \impl \bbB$ and free functions $\lambda^\#_q: \bbN \impl
%% \bbN$, which are defined such that (i) $\lambda^\bbB_q(t)$ is true iff there is a
%% path $\sigma$ from an initial state of the LTS to $t$ such that $q$ is included
%% in the state of $\mU$ after reading $\sigma$, and (ii) valuations of the
%% $\lambda^\#_q$ must be increasing along paths of $\mU$, and strictly increasing
%% for transitions that enter a rejecting state of $\mU$. Together, this ensures
%% that an LTS satisfying these constraints cannot have runs which enter rejecting
%% states infinitely often (and thus would be rejected by $\mU$).

\subsubsection*{Step 3: Solving, Iteration for Increasing Bounds}
%To obtain a decidable problem, we restrict the number of states in the
%LTS that we are looking for, which allows us to instantiate all quantifiers over
%state variables $t,t'$ explicitly with all values in the given range. 
The SMT constraints from step $2$ are 
%in the theory of linear arithmetic with free function symbols. They are 
decidable because the state set and the number of inputs to each process are bounded. If they are satisfiable, a model of the SMT constraints represents a valid implementation of the system.
%If any of these were unbounded, we would have to use unbounded quantification instead of the finite conjunction in step $2$, making the satisfiability problem undecidable.
%Thus, for a given bound $k$ on the size of the system, satisfiability of the constraints is decidable. 
By increasing the size bound incrementally, a valid implementation will eventually be found, if it exists.
%If the constraints are unsatisfiable for a given bound $k$, we increase $k$, add the necessary formulas to the encoding, and try again. If they are satisfiable, we obtain a model, giving us an implementation for the system processes such that $\spec$ is
%satisfied.

\begin{thm}[\cite{FinkbeinerS13}]
If a given LTL specification $\spec$ is realizable in a given distributed 
architecture $A$, then the bounded synthesis procedure will eventually 
terminate and return 
implementations of the system processes that satisfy $\spec$ in $A$.\footnote{Informally, an architecture defines the number of processes in the system, and their means of communication.}
\end{thm}

\subsection{Adaption to Guarded Protocols}
\label{sec:adapted}

We adapt the bounded synthesis approach for synthesis of guarded protocols 
with the following modifications:
\subsubsection*{Interleaving, Non-Determinism, Bottom-Up Encoding}
\begin{itemize}
\item Additional constraints ensure interleaving semantics of the 
resulting system.
\item We use a transition \emph{relation} instead of a function, as our 
systems are inherently non-deterministic.\sj{add explanation?}
\item Instead of a global transition relation and projections to the local 
state spaces, we directly encode local transition relations and local state 
labels. In particular, copies of the same template use the same function 
symbols.
\end{itemize}
\subsubsection*{Guard Assignment and Evaluation}
We encode the valuation of guard variables and guards as defined in Section~\ref{sec:model}. For the guard assignment functions, we introduce (for every process template $U$) additional free function symbols $\guard_U:T_U \times \bbB^E \times T_U \rightarrow \bbB^G$, to be synthesized based on their relation to the local transition relation $\delta_U$.
\sj{explain encoding/evaluation of guards?}
\subsubsection*{Optional: Increasing Set of Guard Variables}
In the usual system model of guarded protocols, there are representative 
guard variables for every state of every process template, whereas we 
generally only consider a partially informed setting where guard variables 
only represent a fixed set of observable states. 
To support the fully-informed case, we optionally add state labels and re-
compute the set of guard variables whenever the size bound on process 
templates changes.
%\subsubsection*{Ensuring Input-independent Enabledness}
%We require that, for every global state and every environment input, if there is an enabled transition, then there must exist an enabled transition for \emph{every} environment input:
%\[ \begin{array}{l}
%\forall s \in S.\ \forall t' \in T\ \forall e \in E.\\
%\left(\begin{array}{l}
%\eval(\guard(s^p,e,t'),g(s,p)) \rightarrow \\
%\qquad \forall e' \in E\ \exists t'' \in T.\ \eval(\guard(s^p,e',t''),g(s,p))
%\end{array}\right)
%\end{array} \]
 
\subsubsection*{Encoding Strong Fairness and Absence of Local Deadlocks}
For specifications $\spec$ that include liveness properties, we synthesize the system under additional fairness assumptions, as discussed in Section~\ref{sec:fairness}. The resulting specification is: 
% \begin{align*}
\[\begin{array}{ll}
& (\forall{i}. \GF (\neg \enabled_i \lor \sched_i)) \impl (\forall{i}.\GF\enabled_i) \\
\land & (\forall{i}. \GF \sched_i) \impl \spec.
\end{array}
\]
% \end{align*} 

\subsection{Correctness of Bounded Template Synthesis}
Based on correctness of the original bounded synthesis approach (and correct
modeling of the features of guarded protocols), we obtain soundness and completeness of bounded template synthesis:
 
\begin{cor}
\label{cor:synthesis:correctness}
If a given specification $\spec$ is realizable in a (disjunctive/conjunctive) 
guarded protocol with process multiplicities $(n_1,n_2)$, then the 
bounded template synthesis procedure will eventually terminate and return 
process templates $(U_1, U_2)$, with $(U_1, U_2)^{(n_1, n_2)} \models \spec$.
\end{cor}

%
The given procedure
will not terminate if the specification is unrealizable.
Since the distributed realizability problem is in general 
undecidable~\cite{Pnueli90,Schewe06,Schewe13},
there is no algorithm that can
detect distributed unrealizability in all cases. We conjecture the same is 
the case for the template realizability problem.


==> experiments-20150205.tex <==
\section{Experiments}
\label{sec:experiments}

We used our new cutoff results in the context of parameterized synthesis to 
automatically construct guarded protocols with safety and lifeness guarantees 
for systems with an arbitrary number of components.
Our prototype is an extension of the parameterized synthesis tool {\sc Party}~\cite{Khalimov13a}.
It synthesizes guarded protocols using the following loop, for increasing 
bounds $(\bound_A,\bound_B)$ on the size of process templates:
\begin{enumerate}
\item[0.] initialize: set $(\bound_A,\bound_B)=(2,2)$
\item \label{enum:experimentsAlgorithm:propertyInst} automatically detect 
cutoff and instantiate specification
\item \label{enum:experimentsAlgorithm:ltl3ba} convert $\LTLmX$ specification into automaton
\item \label{enum:experimentsAlgorithm:enc} encode bounded template synthesis problem into SMT, check satisfiability
\item if SAT: return model of process templates; else increase $(\bound_A,\bound_B)$ and goto 1
% \begin{itemize}[leftmargin=*]
% \item if SAT, convert SMT model into process templates
% \item if UNSAT, increase size bound and goto 1
% \end{itemize}
\end{enumerate}
%
%In the cutoff detection step, we apply the cutoff results from 
%Section~\ref{sec:cutoffs} modularly, i.e., we calculate cutoffs and convert 
%to universal co-Büchi tree automaton (UCT)\sj{remind/use long version} for every conjunct of the specification separately (an optimization 
%mentioned in~\cite{KhalimovJB13b}). Finally, we produce the SMT encoding, 
%conjoining the SMT constraints for all parts. 
%
The method supports modular application of cutoffs for different properties and deadlock detection (cf. \cite{KhalimovJB13b}). For our evaluation, we selected one example for each guard type, and synthesized valid implementations, starting from an initial size bound of 2 for each template. 
%We analyzed the impact of cutoffs by comparing the algorithm's runtime for synthesis with and without cutoffs with respect to an increasing number of instances. In both cases, we used the symmetry observation for encoding the properties, e.g., in a system with 4 processes the property $\bigwedge_i \always(r_i \rightarrow \eventually g_i)$ is instantiated to $\always(r_1 \rightarrow \eventually g_1)$ instead of  $\always(r_1 \rightarrow \eventually g_1) \wedge \dots \wedge \always(r_4 \rightarrow \eventually g_4)$. \sa{Label vs. state -- should be no difference here}
The experiments were done on a Linux machine with a 3.5GHz Intel i7 CPU and 4GB RAM, where a single core was assigned to the synthesis task. Table~\ref{table:experimentsRuntimes} provides the runtimes resulting from our experiments.
We observe for each guard type that the runtime increases rapidly regarding the system size $n$. Applying cutoffs entails an upper bound for the the runtime, making the synthesis of large systems feasible. 

%\begin{table}
%\centering
%\caption{Impact of using cut-offs on synthesis runtime $[s]$, timeout=90min.}
%\label{table:experimentsRuntimes}
%\begin{tabular}{c|c|c|c|c|c|c|}
    %& \multicolumn{2}{c|}{\multirow{2}{*}{Disjunctive Guards}} & \multicolumn{4}{c|}{Conjunctive Guards} \\
%% 		\cline{4-9}
    %& \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{Example 1} & \multicolumn{2}{c|}{Example 2} \\\hline
%$n$ & w/o cut-offs & with cut-offs & w/o cut-offs & with cut-offs & w/o cut-offs & with cut-offs \\\hline
%% 1 & $2.0$   & $2.0$     & $-$    & $-$     \\\hline         & $-$      \\\hline        
%2 & \multicolumn{2}{c|}{1.52}      & \multicolumn{2}{c|}{2.08}  & \multicolumn{2}{c|}{26.6}   \\\hline 
%3 & \multicolumn{2}{c|}{4.1}       & 8.79    & 4.83     & \multicolumn{2}{c|}{590.5}   \\\hline
%4 & \multicolumn{2}{c|}{12.1}      & 42.2    & 4.83    & TIMEOUT & 2819.2  \\\hline
%5 & 41.18    & 41.18              & 230     & 4.83    & TIMEOUT & 2819.2  \\\hline
%6 & 149.83    & 41.18              & 2113    & 4.83    & TIMEOUT & 2819.2  \\\hline
%7 & 481.06    & 41.18              & TIMEOUT & 4.83    & TIMEOUT & 2819.2  \\\hline
%8 & 1650      & 41.18              & TIMEOUT & 4.83    & TIMEOUT & 2819.2  \\\hline
%9 & TIMEOUT   & 41.18              & TIMEOUT & 4.83    & TIMEOUT & 2819.2  \\\hline
%\end{tabular}
%%\vspace{-13pt}
%\end{table}

\begin{figure}[Htb]
\centering
\subfloat[Impact of using cut-offs on synthesis runtime s, timeout=90min.]{
%\centering
\makebox[0.45\textwidth][c]{
\scalebox{0.85}{
\centering
\begin{tabular}{c|c|c|c|c|}
    & \multicolumn{2}{c|}{\multirow{2}{*}{Disjunctive Guards}} & \multicolumn{2}{c|}{Conjunctive Guards} \\
% 		\cline{4-9}
$n$ & w/o cut-offs & with cut-offs & w/o cut-offs & with cut-offs \\\hline
% 1 & $2.0$   & $2.0$     & $-$    & $-$     \\\hline         & $-$      \\\hline        
2 & \multicolumn{2}{c|}{1.53}      & \multicolumn{2}{c|}{8.78}   \\\hline 
3 & \multicolumn{2}{c|}{8.42}      & \multicolumn{2}{c|}{65.34}   \\\hline
4 & \multicolumn{2}{c|}{80}        & TIMEOUT & 1085.8 \\\hline
5 & \multicolumn{2}{c|}{TIMEOUT}   &  \multicolumn{2}{c|}{TIMEOUT} \\\hline
6 & \multicolumn{2}{c|}{TIMEOUT}   & \multicolumn{2}{c|}{TIMEOUT}  \\\hline
7 & \multicolumn{2}{c|}{TIMEOUT}   & \multicolumn{2}{c|}{TIMEOUT}  \\\hline
8 & \multicolumn{2}{c|}{TIMEOUT}   & \multicolumn{2}{c|}{TIMEOUT}  \\\hline
9 & \multicolumn{2}{c|}{TIMEOUT}   & \multicolumn{2}{c|}{TIMEOUT}  \\\hline
\end{tabular}}
\label{table:experimentsRuntimes}
}}
%\qquad
%\subfloat[Example 2]{
%\makebox[0.28\textwidth][c]{
%\scalebox{0.85}{\input{img/mutual_exclusion2_lts}}
%\label{fig:conjunctiveLTS2}
%}}
\qquad
\subfloat[Runtime Chart]{
\makebox[0.45\textwidth][c]{
\raisebox{-6em}{\scalebox{0.20}{\includegraphics{img/experiments.pdf}}}
\label{fig:conjunctiveLTS3}
}}
%
\end{figure}


%\begin{table}
%\centering
%\caption{Impact of synthesizing label-based guards on runtime of conjunctive guards synthesis $[s]$, timeout=90min.}
%\label{table:experimentsGuardTypeRuntimes}
%\begin{tabular}{c|c|c}
%$n$  & state guards    & label guards  \\\hline
%% 1    & $-$             & $-$           \\\hline
%2    & $10.7$          & $8.5$         \\\hline
%3    & $1090$          & $79.3$        \\\hline
%4    & TIMEOUT         & $1040$        \\\hline
%% 5    & TIMEOUT         & TIMEOUT       \\\hline
%\end{tabular}
%\end{table}

\smartpar{Disjunctive Guards.}
We want to obtain a closed system $\largesys$, where $A$ controls an output signal $w$, and every $B^i$ a signal $g_i$. 
The specification is 
$\GF(\neg w) \wedge \GF w \wedge \bigwedge_{i} \left[\GF(w \wedge g_i) \wedge  \GF g_i \wedge \GF(\neg g_i) \right]$ under fair scheduling, i.e., all processes most toggle their signals infinitely often, and every process $B^i$ must ``meet'' infinitely often with $A$ when both signals are enabled.
%  
%\begin{figure}[ht]
%\vspace{-10pt} 
%\centering
%\scalebox{0.75}{\input{img/disjunctive_lts}}
%\caption{Example: Disjunctive Guarded Implementation}
%\label{fig:disjunctiveLTS}
%\vspace{-10pt} 
%\end{figure}
\rb{bad name $a^1$? you use it to denote $i$th process} \sj{make it $1_A$, $2_A$, $1_B$, \ldots?}
Figure~\ref{fig:disjunctiveLTS} shows an implementation synthesized.
For this example, the cutoff for deadlock detection is $5$, and the cutoff for the $\LTLmX$-property is $6$. \rb{why? -- mistake, also explain} \sa{corrected}. Accordingly, Table~\ref{table:experimentsRuntimes} shows that cutoffs do not improve runtimes for systems with $n\leq 5$, but for $n \ge 5$ the cutoff approach has a constant runtime, since the generated templates are guaranteed to be correct for any bigger system.
\rb{example is not realistic -- is there a more realistic?} \sa{Unfortunately, we have a timeout before any cutoff comes into play.}


\smartpar{Conjunctive Guards.}\rb{add `Fair'?}
We want to obtain fair open systems $(B)^{(n)}$ with a single process template $B$ (i.e., $A$ can be arbitrary and $B$ does not react to it), based on the example mentioned in the introduction.
In the specification, each $B^i$ has input $r_i$\rb{$r^i$?} (`request') and output $g_i$ (`grant'). 
The specification requires: i) `every request should be granted', ii) `there should be no spurious grants', iii) mutual exclusion of grants, and iv) before granting, the process enters a trying state. To make the trying state observable, each process has an additional output $t_i$ that is raised if the process is in the trying state.
% Each process must respond to a request by finally setting the grant signal. 
% Besides guaranteeing mutual exclusion, spurious grants must be prevented.
% \begin{align*}
% &\bigwedge_i \always(r_i \wedge \sched_i \rightarrow \eventually g_i) \wedge \bigwedge_{i \neq j} \always(\neg(g_i \wedge g_j))\, \wedge\\ 
% &\bigwedge_i \always\left[g_i \rightarrow g_i \until (\neg g_i \weakuntil (r_i \wedge \sched_i))\right] \wedge\\
% &\bigwedge_i \neg\left[(\neg r_i \wedge \neg g_i) \until (\neg r_i \wedge g_i)\right]
% \end{align*}
% Predicate $\sched_i$ is used to specify that only requests which can be recognized by the process (i.e., if the process is scheduled) need to be granted.
% 
% \begin{figure}[ht]
%\begin{figure}[Htb]
%\centering
%\subfloat[Example 1]{
%\centering
%\makebox[0.29\textwidth][c]{
%\scalebox{0.85}{\input{img/mutual_exclusion_lts}}
%\label{fig:conjunctiveLTS1}
%}}
%%\qquad
%%\subfloat[Example 2]{
%%\makebox[0.28\textwidth][c]{
%%\scalebox{0.85}{\input{img/mutual_exclusion2_lts}}
%%\label{fig:conjunctiveLTS2}
%%}}
%\qquad
%\subfloat[Example 2]{
%\makebox[0.28\textwidth][c]{
%\scalebox{0.85}{\input{img/mutual_exclusion3_lts}}
%\label{fig:conjunctiveLTS3}
%}}
%%
%\caption{Conjunctive Guarded Implementations}
%\label{fig:conjunctiveLTS}
%\end{figure}
\begin{figure}[Htb]
\subfloat[Disjunctive Guarded Implementation]{
\centering
\makebox[0.6\textwidth][c]{
\scalebox{0.85}{\input{img/disjunctive_lts}}
\label{fig:disjunctiveLTS}
}}
\qquad
\subfloat[Conjunctive Guarded Implementation]{
\centering
\makebox[0.29\textwidth][c]{
\scalebox{0.85}{\input{img/mutual_exclusion_trying}}
\label{fig:conjunctiveLTS1}
}}
%
\caption{Example Implementations}
\label{fig:examples}
\end{figure}
Figure~\ref{fig:conjunctiveLTS1} shows an implementation synthesized.
%$t_0$ denotes the initial state. Consider a certain process $i$. Whenever the process is scheduled and the request signal $r_i$ is set, the transition to state $t_1$ is enabled. Thus, the process moves to $t_1$ and remains in this state as long as the guard $\{t_0, t_1\}$ is not satisfied, i.e., if there is at least on other process in the critical state $t_2$. Eventually all other processes are either in $t_0$ or in $t_1$, and process $i$ moves from $t_1$ to $t_2$, thus grants the request it received in state $t_0$. The grant signal $g_i$ is set until process $i$ is scheduled again, then it moves back to the initial state, where $g_i$ is false. The example requires at least three states. %\sa{Insert graph here}
%We managed to synthesize this under the following conditions: \ldots
For this example, the cutoff for properties is $ \leq 3$, and for local deadlock detection it is $4$ (for implementations of size $3$). Accordingly, the table shows some benefit of the cutoff method already for $n=4$.

%The second example defines one request signals $r$, and a two grant signals $g_1$, and $g_2$. The properties are as follows: i) `every request $r$ should finally be granted by $g_1$, followed by $g_2$', ii) `there should be no spurious grants', iii) `mutual exclusion of grants'.
%%
%Figure~\ref{fig:conjunctiveLTS2} shows an implementation synthesized. The cutoff for single-indexed and double-indexed properties is 1, and 2, respectively. The deadlock detection cutoff is $c=3$.

\rb{not clear -- how is this parameterized?}%The second example defines two request signals $r_1$, $r_2$, and a two grant signals $g_1$, and $g_2$. The properties are as follows: i) `every request $r_1$ should eventually be granted ($g_1$)', ii) `every request $r_2$ should eventually be granted ($g_2$) unless resource 1 is requested ($r_1$)', iii) `there should be no spurious grants', iv) `mutual exclusion of grants'. Figure~\ref{fig:conjunctiveLTS3} shows an implementation which satisfies the given specification. As before, we modularly use the cutoff $3$ for properties, and $4$ for deadlock detection. Note that we do not restrict synthesis to $1$-guarded processes, and therefore the cutoff does not guarantee absence of local deadlocks (although manual inspection shows that local deadlocks are not possible with the resulting implementation).

%Finally, we compared the performance of the synthesis algorithm wrt. guards based on i) labels and ii) on states, as mentioned in Section~\ref{sec:adapted}. We observed a speed-up of an order of magnitude when only considering label-based guards, but thus far have only evaluated it on the single example above.

% we analyzed the impact of the optional optimization mentioned in Section~\ref{sec:adapted}, comparing the performance of our synthesis algorithm regarding guards based on labels and guards based on states. 
% The runtime results in  show significant speed-ups, albeit we have thus far only tested the optimization for this single example. %By contrast, we do not profit from this optimization if the number of possible label assignments exceeds the number of states.


==> experiments-full.tex <==
\section{Implementation and Experiments}
\label{sec:experiments}

We implemented our synthesis approach based on {\sc Party}~\cite{Khalimov13a}, 
a tool for parameterized synthesis of token rings. Our tool is written in 
Python and inherits from {\sc Party} the specification language and 
interfaces to automata translation tool LTL3BA~\cite{BabiakKRS12}. For generating and solving the SMT problem, we use the Python API of the solver Z3~\cite{Moura08}.

We synthesize guarded protocols using the following loop, for increasing 
bounds on the size of process templates:
\begin{enumerate}
\item \label{enum:experimentsAlgorithm:propertyInst} automatically detect 
cutoff and instantiate specification
\item \label{enum:experimentsAlgorithm:ltl3ba} call LTL3BA to convert 
specification into automaton
\item \label{enum:experimentsAlgorithm:enc} produce SMT encoding of bounded 
synthesis problem
\item call Z3: 
if SAT, return the model for process templates, else if UNSAT increase size bound and goto 1
% \begin{itemize}[leftmargin=*]
% \item if SAT, convert SMT model into process templates
% \item if UNSAT, increase size bound and goto 1
% \end{itemize}
\end{enumerate}

In the cutoff detection step, we apply the cutoff results from 
Section~\ref{sec:cutoffs} modularly, i.e., we calculate cutoffs and convert 
to universal co-Büchi tree automaton (UCT)\sj{remind/use long version} for every conjunct of the specification separately (an optimization 
mentioned in~\cite{KhalimovJB13b}). Finally, we produce the SMT encoding, 
conjoining the SMT constraints for all parts.

For our evaluation, we selected one example for each guard type, and synthesized valid implementations, starting from an initial bound of 2 for each template. We analyzed the impact of cutoffs by comparing the algorithm's runtime for synthesis with and without cutoffs with respect to an increasing number of instances. In both cases, we used the symmetry observation for encoding the properties, e.g., in a system with 4 processes the property $\bigwedge_i \always(r_i \rightarrow \eventually g_i)$ is instantiated to $\always(r_1 \rightarrow \eventually g_1)$ instead of  $\always(r_1 \rightarrow \eventually g_1) \wedge \dots \wedge \always(r_4 \rightarrow \eventually g_4)$. \sa{Label vs. state -- should be no difference here}

The experiments were done on a Linux machine with a 3.5GHz Intel i7 CPU and 4GB RAM, where a single core was assigned to the synthesis task. Table~\ref{table:experimentsRuntimes} provides the runtimes resulting from our experiments.
\sj{table needs to be explained, or removed}
We observe for each guard type that the runtime increases rapidly regarding the system size $n$. Applying cutoffs entails an upper bound for the the runtime, making the synthesis of large systems feasible. This upper bound is reached for system size $n=2$ and $n=4$ for the conjunctive guarded system, respectively, and system size $n=4$ for disjunctive guarded system. Moreover, we observe that applying cutoffs yields a runtime reduction for $n \geq 2$ in case of our conjunctive guarded system, and $n=4$ in case of disjunctive guarded system.

\begin{table}
\centering
\caption{Impact of using cut-offs on runtime $[s]$, timeout=90min.\sa{TODO}}
\label{table:experimentsRuntimes}
\begin{tabular}{c|c|c|c|c|c|c|c|c}
    & \multicolumn{2}{c|}{\multirow{2}{*}{Disjunctive Guards}} & \multicolumn{4}{c}{Conjunctive Guards} \\\cline{4-9}
    & \multicolumn{2}{c|}{} & \multicolumn{2}{c|}{Example 1} & \multicolumn{2}{c}{Example 2} & \multicolumn{2}{c}{Example 3} \\\hline
$n$ & w/o cut-offs & with cut-offs & w/o cut-offs & with cut-offs & w/o cut-offs & with cut-offs & w/o cut-offs & with cut-offs \\\hline
% 1 & $2.0$   & $2.0$     & $-$    & $-$     \\\hline         & $-$      \\\hline        
2 & \multicolumn{2}{c|}{1.52}      & 2.08    & 0.99   & 5.75    & 5.75  & 26.6    & 12.1   \\\hline 
3 & \multicolumn{2}{c|}{4.1}       & 8.79    & 0.99   & 88.3    & 18.7  & 590.5   & 40.4   \\\hline
4 & \multicolumn{2}{c|}{12.1}      & 42.2    & 0.99   & 369.3   & 105.1 & TIMEOUT & 219.2  \\\hline
5 & 41.177    & 23.15              & 230     & 0.99   & 3240    & 105.1 & TIMEOUT & 219.2  \\\hline
6 & 149.83    & 23.15              & 2113    & 0.99   & TIMEOUT & 105.1 & TIMEOUT & 219.2  \\\hline
7 & 481.06    & 23.15              & TIMEOUT & 0.99   & TIMEOUT & 105.1 & TIMEOUT & 219.2  \\\hline
8 & 1650      & 23.15              & TIMEOUT & 0.99   & TIMEOUT & 105.1 & TIMEOUT & 219.2  \\\hline
9 & TIMEOUT   & 23.15              & TIMEOUT & 0.99   & TIMEOUT & 105.1 & TIMEOUT & 219.2  \\\hline
\end{tabular}
%\vspace{-13pt}
\end{table}

%\begin{table}
%\centering
%\caption{Impact of synthesizing label-based guards on runtime of conjunctive guards synthesis $[s]$, timeout=90min.}
%\label{table:experimentsGuardTypeRuntimes}
%\begin{tabular}{c|c|c}
%$n$  & state guards    & label guards  \\\hline
%% 1    & $-$             & $-$           \\\hline
%2    & $10.7$          & $8.5$         \\\hline
%3    & $1090$          & $79.3$        \\\hline
%4    & TIMEOUT         & $1040$        \\\hline
%% 5    & TIMEOUT         & TIMEOUT       \\\hline
%\end{tabular}
%\end{table}


\subsection{Disjunctive Guards}

We consider instances of a closed system $(U_1, U_2)^{(1, n)}$. The first process template has an output signal $w$, the second -- $g$. 
The specification is 
$\GF(\neg w) \wedge \GF w \wedge \bigwedge_{i} \left[\GF(w \wedge g_i) \wedge  \GF g_i \wedge \GF(\neg g_i) \right]$.
%  
\begin{figure}[ht]
\vspace{-10pt} 
\centering
\scalebox{0.75}{\input{img/disjunctive_lts}}
\caption{Example: Disjunctive Guarded Implementation}
\label{fig:disjunctiveLTS}
\vspace{-10pt} 
\end{figure}
Figure~\ref{fig:disjunctiveLTS} shows an implementation synthesized.
For this example, the deadlock detection cutoff for $U_2$ is $3$. Cutoffs for single-indexed and double-indexed properties of the specification are $4$.
Therefore, we observe no runtime differences when comparing synthesis with cutoffs and synthesis without cutoffs for $n \leq 3$ instances of $U_2$ (see Table~\ref{table:experimentsRuntimes}). For $n=4$, the deadlock detection cutoff causes a runtime improvement. The maximum cutoff $c=4$ enables us to successfully synthesize systems for an arbitrary number of $U_2$ instances.
%The states $a^0$ and $b^0$ are the initial states of templates $U_1$ and $U_2$, while the states $a^1$ and $b^1$ are the respective synchronization states. Process $U_1
%One the one hand, process $U_1^1$ can enter its synchronization state $t_1^1$ without any restrictions, but can only move back to the initial state if there is at least one instance of $U_2$ in a synchronization state $t_2^1$. On the other hand, $U_2$ processes can only move if the $U_1$ process is in its synchronization state. Thus, there must be at least one pair-wise synchronization every time the $U_1$ process enters $t_1^1$.  \sa{Description of templates necessary?}
%We managed to synthesize this under the following conditions: \ldots \sa{Insert graph here}

\subsection{Conjunctive Guards}
We consider a system $(U)^{(n)}$ with a single process template\ak{r u sure that cutoffs stay for one-template systems?}. We analyze the synthesis results for three different specifications.

In the first specification, each process has input $r$ (`request') and output $g$ (`grant'). 
The specification requires: i) `every request should be granted', ii) `there should be no spurious grants', and iii) mutual exclusion of grants. 
% Each process must respond to a request by finally setting the grant signal. 
% Besides guaranteeing mutual exclusion, spurious grants must be prevented.
% \begin{align*}
% &\bigwedge_i \always(r_i \wedge \sched_i \rightarrow \eventually g_i) \wedge \bigwedge_{i \neq j} \always(\neg(g_i \wedge g_j))\, \wedge\\ 
% &\bigwedge_i \always\left[g_i \rightarrow g_i \until (\neg g_i \weakuntil (r_i \wedge \sched_i))\right] \wedge\\
% &\bigwedge_i \neg\left[(\neg r_i \wedge \neg g_i) \until (\neg r_i \wedge g_i)\right]
% \end{align*}
% Predicate $\sched_i$ is used to specify that only requests which can be recognized by the process (i.e., if the process is scheduled) need to be granted.
% 
% \begin{figure}[ht]
\begin{figure}[Htb]
\centering
\subfloat[Example 1]{
\centering
\makebox[0.29\textwidth][c]{
\scalebox{0.85}{\input{img/mutual_exclusion_lts}}
\label{fig:conjunctiveLTS1}
}}
\qquad
\subfloat[Example 2]{
\makebox[0.28\textwidth][c]{
\scalebox{0.85}{\input{img/mutual_exclusion2_lts}}
\label{fig:conjunctiveLTS2}
}}
\qquad
\subfloat[Example 3]{
\makebox[0.28\textwidth][c]{
\scalebox{0.85}{\input{img/mutual_exclusion3_lts}}
\label{fig:conjunctiveLTS3}
}}
%
\caption{Conjunctive Guarded Implementations}
\label{fig:conjunctiveLTS}
\end{figure}

Figure~\ref{fig:conjunctiveLTS1} shows an implementation synthesized.
%$t_0$ denotes the initial state. Consider a certain process $i$. Whenever the process is scheduled and the request signal $r_i$ is set, the transition to state $t_1$ is enabled. Thus, the process moves to $t_1$ and remains in this state as long as the guard $\{t_0, t_1\}$ is not satisfied, i.e., if there is at least on other process in the critical state $t_2$. Eventually all other processes are either in $t_0$ or in $t_1$, and process $i$ moves from $t_1$ to $t_2$, thus grants the request it received in state $t_0$. The grant signal $g_i$ is set until process $i$ is scheduled again, then it moves back to the initial state, where $g_i$ is false. The example requires at least three states. %\sa{Insert graph here}
%We managed to synthesize this under the following conditions: \ldots
The evaluation results for conjunctive guarded systems show that the bound independent property cutoffs are of benefit for the runtime also if small systems are synthesized. Also, the problem complexity does not increase if additional processes are added to systems of size $n\geq 3$, the deadlock-detection cutoff. \sa{Compare to mutual exclusion without spurious.}
The runtime improvement for $n=2$ is due to the modularly applied constant cutoffs for single-indexed ($c=1$), and double-indexed properties 
($c=2$), respectively (see Lemma~\ref{le:FairConjunctiveBounding Lemma}).
%

The second example defines one request signals $r$, and a two grant signals $g_1$, and $g_2$. The properties are as follows: i) `every request $r$ should finally be granted by $g_1$, followed by $g_2$', ii) `there should be no spurious grants', iii) `mutual exclusion of grants'.
%
Figure~\ref{fig:conjunctiveLTS2} shows an implementation synthesized. The cutoff for single-indexed and double-indexed properties is 1, and 2, respectively. The deadlock detection cutoff is $c=3$.

The third example defines two request signals $r_1$, $r_2$, and a two grant signals $g_1$, and $g_2$. The properties are as follows: i) `every request $r_1$ should finally be granted ($g_1$)', ii) `every request $r_2$ should finally be granted ($g_2$) unless resource 1 is requested ($r_1$)', iii) `there should be no spurious grants', `mutual exclusion of grants'. Figure~\ref{fig:conjunctiveLTS3} shows an implementation which satisfies the given specification. As before, we use the constant cutoffs for single-indexed and double-indexed properties, and the deadlock detection cutoff $c=3$.

%Finally, we compared the performance of the synthesis algorithm wrt. guards based on i) labels and ii) on states, as mentioned in Section~\ref{sec:adapted}. We observed a speed-up of an order of magnitude when only considering label-based guards, but thus far have only evaluated it on the single example above.

% we analyzed the impact of the optional optimization mentioned in Section~\ref{sec:adapted}, comparing the performance of our synthesis algorithm regarding guards based on labels and guards based on states. 
% The runtime results in  show significant speed-ups, albeit we have thus far only tested the optimization for this single example. %By contrast, we do not profit from this optimization if the number of possible label assignments exceeds the number of states.


==> img/conj_deadlock_cutoff.tex <==
\begin{tikzLTS}
      \tikzstyle{state} = [circle,draw=black,thick,inner sep=1.5pt, text width={width("$\text{T}_{i-1}$")}, align=center]
      \tikzstyle{boxLabel} = [yshift=-0.4cm]
      \tikzstyle{every node} = [node distance=3cm]

  \node[state] (A) [] {$\text{init}$};
  \node[] (B) [below of=A, node distance=2.5cm] {$$};
  \node[state] (C) [left of=B, node distance=3.5cm] {$1$};
  \node[state] (D) [right of=C] {$2$};
  \node[] (B) [below of=A] {$$};
  \node[] (E) [right of=D] {$$};
  \node[] (E') [below of=E,node distance=0.75cm] {$$};
  \node[node distance=1cm] (F) [right of=E] {$$};
  \node[state] (G) [right of=F] {$n$};
  
\pgfmathsetmacro{\shift}{0.3ex}

\draw [post] (A.185) -- node[above] {} (C.80);
\draw [pre] (A.210) -- node[below right] {$\neg 1$} (C.55);

\draw [post] (A.245) -- node[above] {} (D.90);
\draw [pre] (A.270) -- node[below right] {$\neg 2$} (D.65);

\draw [post] (A.325) -- node[above] {} (G.150);
\draw [pre] (A.350) -- node[above right] {$\neg n$} (G.125);
  
  \path (C) edge [right,post] node [above] {$\neg 2$} (D);
  \path (D) edge [right,post] node [above] {$\neg 3$} (E);
  \path ($(E)-(0.05,0)$) edge [right,dotted,-] node [above] {} ($(F)+(0.05,0)$);
  \path (F) edge [right,post] node [above] {$\neg n$} (G);
  
  \path (G) edge [bend left,post] node [above] {$\neg 1$} (C);
  
   \node (U2) [draw=black, fit=(A) (C) (G) (E'), inner sep=0.75cm] {};
   \node [boxLabel] at (U2.north) {Template $B$};
\end{tikzLTS}

==> img/disj_tight_propA_tmplA.tex <==
%!TEX root = table.tex
\begin{tikzpicture}[node distance=2cm,inner sep=1pt,minimum size=0.5mm,->,>=latex]


\node[state,double] (a_1) {$a_1$};
\node (dots) [right of=a_1] {$\ldots$};
\node[state] (a_n) [right of=dots] {$a_{all}$};


\path (a_1) edge [above] node {$\disj{b_1}$} (dots);
\path (dots) edge [above] node {$\disj{b_{|T_B|}}$} (a_n);



\end{tikzpicture}


==> img/disj_tightness_fair_prop.tex <==
\begin{tikzLTS}
      \tikzstyle{state} = [circle,draw=black,thick,inner sep=1.5pt, text width={width("$\text{init}_1$")}, align=center]
      \tikzstyle{boxLabel} = [yshift=-0.4cm]

    \newcommand{\rad}{2 }
    \draw[draw=white] (0,0) circle (3);
    \foreach \x[remember=\x as \lastx] in {1,2,...,5}{
      \ifnum \x < 4
      \node[state] (t\x) at ($(0,0)+({-72*(\x-2)+18}:\rad and \rad)$) {$a_\x$};
      \else
       \ifnum \x = 4
         \coordinate (t\x) at ($(0,0)+({-72*(\x-2)+18}:\rad and \rad)$) ;
        \else
         \node[state] (t\x) at ($(0,0)+({-72*(\x-2)+18}:\rad and \rad)$) {$a_{|T_B|}$};
        \fi
      \fi
    }

    \coordinate (t34) at ($(0,0)+({-72*(4-2)+36}:\rad and \rad)$) ;
    \coordinate (t44) at ($(0,0)+({-72*(4-2)-0}:\rad and \rad)$) ;

      \path (t1) [post,bend left] edge node[above right] {$\disj{b_1}$} (t2);
      \path (t2) [post,bend left] edge node[below right] {$\disj{b_2}$} (t3);
      \path (t3) [post,bend left,dashed] edge node[below] {$\disj{b_3}$} (t34);
      \path (t34) [bend left,dotted] edge (t44);
      \path (t44) [post,bend left,dashed] edge node[above right] (e34-44) {$\disj{b_{|T_B|-1}}$} (t5);
      \path (t5) [post,bend left] edge node[above left] {\disj{b_{|T_B|}}} (t1);

	 \node (U1) [draw=black, fit=(t1) (t2) (t3) (t4) (t5) (t34) (t44), inner sep=0.75cm] {} ;
	 \node [boxLabel] at (U1.north) {Template $A$};

     \coordinate(tright) at (U1.east);
     %\draw[black] ($(t5.west |- t1.north)-(1, -1)$) rectangle ($(t2.east |- t3.south)+(1,-1)$);
     %\path  ($(t5.west |- t1.north)-(1, -1.1)$) -- ($(t2.east |- t1.north)+(1, 1.1)$) node[midway,above] {$\mathcal{T}_1$};

    \newcommand{\dist}{4 }
    \node[state] (t1) at ($(tright |- t1)+(4,0)$) {$b_1$};
    \node[state] (t2) at ($(tright |- t3)+(\dist/2,0.5)$) {$b_2$};
    \node[state] (t3) at ($(tright |- t3)+(\dist/2+2,0.5)$) {$b_3$};
    \node (ti) at ($(tright |- t3)+(\dist/2+3.5,0)$) {\dots\dots};
    \node[state] (t5) at ($(tright |- t3)+(\dist/2+5,0)$) {$b_k$};

    \path (t1) edge[post,loop left] node[left] {\disj{b_1}} (t1)
              (t1) edge[post]  (t2)
              (t1) edge[post]  (t3)
              (t1) edge[post]  (t5)
%               (t1) edge[post] node[above left] {$|T_B|$} (t2)
%               (t1) edge[post] node[above right] {$|T_B|$} (t3)
%               (t1) edge[post] node[above right] {$|T_B|$} (t5)
              (t2) edge[post,loop below] node[below] {\disj{b_2}} (t2)
              (t3) edge[post,loop below] node[below] {\disj{b_3}} (t3)
              (t5) edge[post,loop below] node[below] {\disj{b_k}} (t5);

	 \coordinate(U1bottom) at ($(t2 |- U1.south)+(0,0.75)$);
     \node (U2) [draw=black, fit=(t1) (t2) (t3) (ti) (t5) (U1bottom), inner sep=0.75cm] {} ;
	 \node [boxLabel] at (U2.north) {Template $B$};;



\end{tikzLTS}

==> img/disj_tightness_fair_prop_run.tex <==
\begin{tikzPath}    
    \node (T21-0) [pstate,label=right:$a_1$] {}; 
    \node (T21-1) [below of=T21-0,hiddenstate,label=right:$$] {};           
    \node (T21-2) [below of=T21-1,pstate,label=right:$a_1$] {};
    \node (T21-3) [below of=T21-2,pstate,label=right:$a_2$] {};           
    \node (T21-4) [below of=T21-3,pstate,label=right:$a_3$] {};
    \node (T21-5) [below of=T21-4,hiddenstate,label=right:$$] {};
        
    \draw[trans-notsched,dashed] (T21-0) -- (T21-2); 
    \draw[trans-notsched] (T21-2) -- (T21-3);
    \draw[trans-notsched] (T21-3) -- (T21-4);
    \draw[trans-notsched] (T21-4) -- (T21-5);
    
    \node (T22-0) [pstate,right of=T21-0,label=right:$b_1$,node distance=1cm] {}; 
    \node (T22-1) [below of=T22-0,hiddenstate,label=right:$$] {};           
    \node (T22-2) [below of=T22-1,hiddenstate,label=right:$$] {};
    \node (T22-3) [below of=T22-2,hiddenstate,label=right:$$] {};           
    \node (T22-4) [below of=T22-3,hiddenstate,label=right:$$] {};
    \node (T22-5) [below of=T22-4,hiddenstate,label=right:$$] {};

    \draw[trans-notsched,dashed] (T22-0) -- (T22-5);
    
    \node (T22-0) [pstate,right of=T22-0,label=right:$b_1$,node distance=1cm] {}; 
    \node (T22-1) [below of=T22-0,hiddenstate,label=right:$$] {};           
    \node (T22-2) [below of=T22-1,hiddenstate,label=right:$$] {};
    \node (T22-3) [below of=T22-2,hiddenstate,label=right:$$] {};           
    \node (T22-4) [below of=T22-3,hiddenstate,label=right:$$] {};
    \node (T22-5) [below of=T22-4,hiddenstate,label=right:$$] {};

    \draw[trans-notsched,dashed] (T22-0) -- (T22-5);

\newcommand{\patht}[2]{
    \node (T22-0) [pstate,right of=T22-0,label=right:$b_1$,node distance=#1] {}; 
    \node (T22-1) [below of=T22-0,hiddenstate,label=right:$$] {};           
    \node (T22-2) [below of=T22-1,pstate,label=right:$#2$] {};
    \node (T22-3) [below of=T22-2,hiddenstate,label=right:$$] {};    
    \node (T22-4) [below of=T22-3,hiddenstate,label=right:$$] {};
    \node (T22-5) [below of=T22-4,hiddenstate,label=right:$$] {};

    \draw[trans-notsched] (T22-0) -- (T22-2);
    \draw[trans-notsched,dashed] (T22-2) -- (T22-5);
}

    \patht{1cm}{b_1}
    \patht{1cm}{b_2}
    \patht{1cm}{b_2}
    \node (T22-0) [hiddenstate,right of=T22-0,label=right:$\dots$,node distance=0.75cm] {}; 
    \patht{1.5cm}{b_{|T_B|}}
    \patht{1cm}{b_{|T_B|}}
    \node (T22-0) [hiddenstate,right of=T22-0,label=right:$\dots\dots$,node distance=1cm] {}; 
    \end{tikzPath}

==> img/fig_conj_deadlock-detection-worst-impl.tex <==
\begin{tikzLTS}
      \tikzstyle{state} = [circle,draw=black,thick,inner sep=1.5pt, text width={width("$\text{T}_{i-1}$")}, align=center]
      \tikzstyle{boxLabel} = [yshift=-0.4cm]
      \tikzstyle{every node} = [node distance=3cm]
    
    \node[] (ti) {$\dots\dots\dots\dots$};
    
    \node[state] (t3) [left of=ti, node distance=2cm] {$b_3$};
    \node[state] (t2) [left of=t3] {$b_2$};
    \node[state] (t4) [right of=ti, node distance=2cm] {$b_{i-1}$};
    \node[state] (t5) [right of=t4] {$b_i$};
    \node[] (tii) [right of=t5, node distance=1.5cm] {$\dots\dots$};

    \node[state] (t1) [above of=ti] {$b_1$};


	\draw (t1) [post, bend right] edge node [above left] (l1) {} (t2);
	\draw (t1) [post] edge node [above left] (l1) {} (t3);
	\draw (t1) [post] edge node [above right] (l1) {} (t4);
	\draw (t1) [post, bend left] edge node [above right] (l1) {} (t5);
	
	\draw (t2) [post, loop above] edge node [above] {$\forall{\neg b_2}$} (t2);
	
	\draw (t2) [post, bend left] edge node [above] {$\forall{\neg b_3}$} (t3);
	\draw (t3) [post, bend left] edge node [below] {$\forall{\neg b_3}$} (t2);
	
	\draw (t4) [post, bend left] edge node [above] {$\forall{\neg b_i}$} (t5);
	\draw (t5) [post, bend left] edge node [below] {$\forall{\neg b_i}$} (t4);

 	 \node (U2) [draw=black, fit=(t1) (t2) (tii), inner sep=0.75cm] {};
 	 \node [boxLabel] at (U2.north) {Template $B$};
\end{tikzLTS}

==> img/fig_conjunctive-deadlock-detection-impossible-comp.tex <==
\begin{tikzPath}	
     	\node (T21-0) [pstate,label=right:$a_1$] {}; 
     	\node (T21-1) [below of=T21-0,hiddenstate,label=right:$$] {};   		
     	\node (T21-2) [below of=T21-1,hiddenstate,label=right:$$] {};
     	\node (T21-3) [below of=T21-2,pstate,label=right:$a_1$] {};   		
	\node (T21-4) [below of=T21-3,pstate,label=right:$a_1$] {};
	    
	\draw[trans-notsched,dashed] (T21-0) -- (T21-3); 
	\draw[trans-notsched] (T21-3) -- (T21-4);
	
     	\node (T22-0) [pstate,right of=T21-0,label=right:$b_1$,node distance=1cm] {}; 
     	\node (T22-1) [below of=T22-0,hiddenstate,label=right:$$] {};   		
     	\node (T22-2) [below of=T22-1,hiddenstate,label=right:$$] {};
     	\node (T22-3) [below of=T22-2,pstate,label=right:$b_1$] {};   		
     	\node (T22-4) [below of=T22-3,pstate,label=right:$b_1$] {};

	\draw[trans-notsched,dashed] (T22-0) -- (T22-3);
	\draw[trans-notsched] (T22-3) -- (T22-4);

\newcommand{\patht}[3]{
     	\node (T22-0) [pstate,right of=T22-0,label=right:$b_1$,node distance=#1] {}; 
     	\node (T22-1) [below of=T22-0,hiddenstate,label=right:$$] {};   		
     	\node (T22-2) [below of=T22-1,hiddenstate,label=right:$$] {};
     	\node (T22-3) [below of=T22-2,pstate,label=right:$#2$] {};
	\node (T22-4) [below of=T22-3,pstate,label=right:$#3$] {};

	\draw[trans-notsched] (T22-0) -- (T22-3);
	\draw[trans-notsched] (T22-3) -- (T22-4);
}

    \patht{1cm}{a_1}{a_1}
    \patht{1cm}{b_2}{b_2}
    \patht{1cm}{b_2}{b_2}
    \node (T22-0) [hiddenstate,right of=T22-0,label=right:$\dots\dots$,node distance=1cm] {}; 
    \patht{2cm}{b_d}{b_d}
    \patht{1cm}{b_d}{b_d}
    \node (T22-0) [hiddenstate,right of=T22-0,label=right:$\dots\dots$,node distance=1cm] {}; 
    \patht{2cm}{b_{|T_B|}}{b_{|T_B|}}
    \patht{1cm}{b_d}{b_{|T_B|}}
    \end{tikzPath}

==> img/fig_disj-bounding_worst-comp.tex <==
\begin{tikzPath}    
    \node (T21-0) [pstate,label=right:$a_1$] {}; 
    \node (T21-1) [below of=T21-0,hiddenstate,label=right:$$] {};           
    \node (T21-2) [below of=T21-1,pstate,label=right:$a_1$] {};
    \node (T21-3) [below of=T21-2,pstate,label=right:$a_2$] {};           
    \node (T21-4) [below of=T21-3,pstate,label=right:$a_3$] {};
    \node (T21-5) [below of=T21-4,hiddenstate,label=right:$$] {};
        
    \draw[trans-notsched,dashed] (T21-0) -- (T21-2); 
    \draw[trans-notsched] (T21-2) -- (T21-3);
    \draw[trans-notsched] (T21-3) -- (T21-4);
    \draw[trans-notsched] (T21-4) -- (T21-5);
    
    \node (T22-0) [pstate,right of=T21-0,label=right:$b_1$,node distance=1cm] {}; 
    \node (T22-1) [below of=T22-0,hiddenstate,label=right:$$] {};           
    \node (T22-2) [below of=T22-1,hiddenstate,label=right:$$] {};
    \node (T22-3) [below of=T22-2,hiddenstate,label=right:$$] {};           
    \node (T22-4) [below of=T22-3,hiddenstate,label=right:$$] {};
    \node (T22-5) [below of=T22-4,hiddenstate,label=right:$$] {};

    \draw[trans-notsched,dashed] (T22-0) -- (T22-5);
    
    \node (T22-0) [pstate,right of=T22-0,label=right:$b_1$,node distance=1cm] {}; 
    \node (T22-1) [below of=T22-0,hiddenstate,label=right:$$] {};           
    \node (T22-2) [below of=T22-1,hiddenstate,label=right:$$] {};
    \node (T22-3) [below of=T22-2,hiddenstate,label=right:$$] {};           
    \node (T22-4) [below of=T22-3,hiddenstate,label=right:$$] {};
    \node (T22-5) [below of=T22-4,hiddenstate,label=right:$$] {};

    \draw[trans-notsched,dashed] (T22-0) -- (T22-5);

\newcommand{\patht}[2]{
    \node (T22-0) [pstate,right of=T22-0,label=right:$b_1$,node distance=#1] {}; 
    \node (T22-1) [below of=T22-0,hiddenstate,label=right:$$] {};           
    \node (T22-2) [below of=T22-1,pstate,label=right:$#2$] {};
    \node (T22-3) [below of=T22-2,hiddenstate,label=right:$$] {};    
    \node (T22-4) [below of=T22-3,hiddenstate,label=right:$$] {};
    \node (T22-5) [below of=T22-4,hiddenstate,label=right:$$] {};

    \draw[trans-notsched] (T22-0) -- (T22-2);
    \draw[trans-notsched,dashed] (T22-2) -- (T22-5);
}

    \patht{1cm}{b_1}
    \patht{1cm}{b_2}
    \patht{1cm}{b_2}
    \node (T22-0) [hiddenstate,right of=T22-0,label=right:$\dots$,node distance=0.75cm] {}; 
    \patht{1.5cm}{b_{|T_B|}}
    \patht{1cm}{b_{|T_B|}}
    \node (T22-0) [hiddenstate,right of=T22-0,label=right:$\dots\dots$,node distance=1cm] {}; 
    \end{tikzPath}

==> img/fig_disj-bounding_worst-comp2.tex <==
\begin{tikzPath}    
    \node (T21-0) [pstate,label=right:$a_1$] {};    
    \node (T21-1) [below of=T21-0,hiddenstate,label=right:$$] {};           
    \node (T21-2) [below of=T21-1,hiddenstate,label=right:$$] {};
    \node (T21-3) [below of=T21-2,hiddenstate,label=right:$$] {};           
    \node (T21-4) [below of=T21-3,hiddenstate,label=right:$$] {};
    \node (T21-5) [below of=T21-4,hiddenstate,label=right:$$] {};
    \draw[trans-notsched,dotted] (T21-0) -- (T21-5);
            
    \node (T22-0) [pstate,right of=T21-0,label=right:$b_1$,node distance=1cm] {}; 
    \node (T22-1) [below of=T22-0,hiddenstate,label=right:$$] {};           
    \node (T22-2) [below of=T22-1,pstate,label=right:$b_1$] {};
    \node (T22-3) [below of=T22-2,hiddenstate,label=right:$$] {};           
    \node (T22-4) [below of=T22-3,pstate,label=right:$b_{|T_B|}$] {};
    \node (T22-5) [below of=T22-4,hiddenstate,label=right:$$] {};

    \draw[trans-notsched,dashed] (T22-0) -- (T22-2);
    \draw[trans-notsched] (T22-2) -- (T22-4);
    \draw[trans-notsched,dashed] (T22-4) -- (T22-5);

\newcommand{\patht}[2]{
    \node (T22-0) [pstate,right of=T22-0,label=right:$b_1$,node distance=#1] {}; 
    \node (T22-1) [below of=T22-0,hiddenstate,label=right:$$] {};           
    \node (T22-2) [below of=T22-1,pstate,label=right:$#2$] {};
    \node (T22-3) [below of=T22-2,hiddenstate,label=right:$$] {};    
    \node (T22-4) [below of=T22-3,hiddenstate,label=right:$$] {};
    \node (T22-5) [below of=T22-4,hiddenstate,label=right:$$] {};

    \draw[trans-notsched] (T22-0) -- (T22-2);
    \draw[trans-notsched,dashed] (T22-2) -- (T22-5);
}

    \patht{1cm}{b_1}
    \patht{1cm}{b_1}
    \patht{1cm}{b_2}
    \patht{1cm}{b_2}
    \node (T22-0) [hiddenstate,right of=T22-0,label=right:$\dots$,node distance=0.75cm] {}; 
    \patht{1.5cm}{b_{|T_B|}}
    %\node (T22-0) [hiddenstate,right of=T22-0,label=right:$\dots$,node distance=1cm] {}; 
    \end{tikzPath}

==> img/fig_disj-bounding_worst-impl.tex <==
\begin{tikzLTS}
      \tikzstyle{state} = [circle,draw=black,thick,inner sep=1.5pt, text width={width("$\text{init}_1$")}, align=center]
      \tikzstyle{boxLabel} = [yshift=-0.4cm]
	  
    \newcommand{\rad}{2 }
    \draw[draw=white] (0,0) circle (3);
    \foreach \x[remember=\x as \lastx] in {1,2,...,5}{
      \ifnum \x < 4
      \node[state] (t\x) at ($(0,0)+({-72*(\x-2)+18}:\rad and \rad)$) {$a_\x$};
      \else
       \ifnum \x = 4
         \coordinate (t\x) at ($(0,0)+({-72*(\x-2)+18}:\rad and \rad)$) ;
        \else
         \node[state] (t\x) at ($(0,0)+({-72*(\x-2)+18}:\rad and \rad)$) {$a_{|T_B|}$};
        \fi
      \fi
    }

    \coordinate (t34) at ($(0,0)+({-72*(4-2)+36}:\rad and \rad)$) ;
    \coordinate (t44) at ($(0,0)+({-72*(4-2)-0}:\rad and \rad)$) ;

      \path (t1) [post,bend left] edge node[above right] {$\disj{b_1}$} (t2);
      \path (t2) [post,bend left] edge node[below right] {$\disj{b_2}$} (t3);
      \path (t3) [post,bend left,dashed] edge node[below] {$\disj{b_3}$} (t34);
      \path (t34) [bend left,dotted] edge (t44);
      \path (t44) [post,bend left,dashed] edge node[above right] (e34-44) {$\disj{b_{|T_B|-1}}$} (t5);
      \path (t5) [post,bend left] edge node[above left] {\disj{b_{|T_B|}}} (t1);
      
	 \node (U1) [draw=black, fit=(t1) (t2) (t3) (t4) (t5) (t34) (t44), inner sep=0.75cm] {} ;
	 \node [boxLabel] at (U1.north) {Template $A$};
	 
     \coordinate(tright) at (U1.east);
     %\draw[black] ($(t5.west |- t1.north)-(1, -1)$) rectangle ($(t2.east |- t3.south)+(1,-1)$);
     %\path  ($(t5.west |- t1.north)-(1, -1.1)$) -- ($(t2.east |- t1.north)+(1, 1.1)$) node[midway,above] {$\mathcal{T}_1$};

    \newcommand{\dist}{4 }
    \node[state] (t1) at ($(tright |- t1)+(4,0)$) {$b_1$};
    \node[state] (t2) at ($(tright |- t3)+(\dist/2,0.5)$) {$b_2$};
    \node[state] (t3) at ($(tright |- t3)+(\dist/2+2,0.5)$) {$b_3$};
    \node (ti) at ($(tright |- t3)+(\dist/2+3.5,0)$) {\dots\dots};
    \node[state] (t5) at ($(tright |- t3)+(\dist/2+5,0)$) {$b_k$};
    
    \path (t1) edge[post,loop left] node[left] {\disj{b_1}} (t1)
              (t1) edge[post]  (t2)
              (t1) edge[post]  (t3)
              (t1) edge[post]  (t5)
%               (t1) edge[post] node[above left] {$|T_B|$} (t2)
%               (t1) edge[post] node[above right] {$|T_B|$} (t3)
%               (t1) edge[post] node[above right] {$|T_B|$} (t5)
              (t2) edge[post,loop below] node[below] {\disj{b_2}} (t2)
              (t3) edge[post,loop below] node[below] {\disj{b_3}} (t3)
              (t5) edge[post,loop below] node[below] {\disj{b_k}} (t5);
    
	 \coordinate(U1bottom) at ($(t2 |- U1.south)+(0,0.75)$);
     \node (U2) [draw=black, fit=(t1) (t2) (t3) (ti) (t5) (U1bottom), inner sep=0.75cm] {} ;
	 \node [boxLabel] at (U2.north) {Template $B$};;
     
  
      
\end{tikzLTS}

==> img/fig_disj-bounding_worst-impl2.tex <==
\begin{tikzLTS}
      \tikzstyle{state} = [circle,draw=black,thick,inner sep=1.5pt, text width={width("$\text{init}_2$")}, align=center]
      \tikzstyle{boxLabel} = [yshift=-0.4cm]
      \tikzstyle{every node} = [node distance=1.75cm]
    
    \node[state] (t1) {$b_1$};
    \node[state] (t2) [below of=t1] {$b_2$};
    \node[] (t3) [below of=t2] {$$};
    \node[] (t4) [below of=t3, node distance=1cm] {$$};
    \node[state] (t5) [below of=t4] {$b_k$};




       \path (t1) [post,loop right] edge node [right] (l1) {$\disj{b_1}$} (t1);
       \path (t1) [post] edge node[right] {$\disj{b_1}$} (t2);
        \path (t2) [post,loop right] edge node [right] (l2) {$\disj{b_2}$} (t2);
        \path (t2) [post,dashed] edge node[right] {$\disj{b_2}$} (t3);
        \path (t3) [dotted] edge (t4);
        \path (t4) [post,dashed] edge node[right] {$\disj{b_{k-1}}$} (t5);
        \path (t5) [post,loop right] edge node[right] (l5) {$\disj{b_k}$} (t5);

  	 \node (U2) [draw=black, fit=(t1) (t2) (t3) (t4) (t5) (l1) (l2) (l5), inner sep=0.75cm] {} ;
 	 \node [boxLabel] at (U2.north) {Template $B$};
\end{tikzLTS}

==> proof-conj-deadlock-global.tex <==
\begin{proof}\ak{remove this proof -- it is kahlon's result and does not have monotonicity.., we have a similar proof in the next theorem}
The result follows from the original proof for global deadlock detection by Emerson and Kahlon~\cite[Lemma 5.2]{Emerson00}. The construction uses two local runs for every $\state \in \stateset_B$ to ensure the global deadlock. We note that processes in the initial state never contribute to a deadlock because of the special form of conjunctive guards. Therefore, it is enough to consider two local runs for every $\state \in \stateset_B \setminus \{\initstate\}$, and the cutoff is $2\card{B}-2$.
\end{proof}

==> proof-disj-bounding.tex <==
\begin{proof}
The following proof is similar to the proof for properties of \emph{closed} disjunctive systems by Emerson and Kahlon~\cite[Lemma 4.1.2]{Emerson00}. We separate the proof into two main constructions that will be re-used in later proofs.

Let $c = \card{B}+2$ and $n \geq c$. In the following, we will call $\largesys$ the \emph{large system}, and $\cutoffsys$ the \emph{cutoff system}.

\medskip
\noindent
Direction $\implies$:\\
Let $x=(s_1,e_1,p_1), (s_2,e_2,p_2) \ldots$ be a run \sj{should runs start with $0$ or $1$?} of $\largesys$ that satisfies $\pexists h(A^1,B^1)$.
In the following, we construct a run $y$ of the cutoff system $\cutoffsys$ such that $y(A^1, B^1)\simeq x(A^1, B^1)$.
Informally, the two steps are the following: 
\begin{enumerate}
  \item \emph{Flooding Construction}:\sj{TODO: separate flooding from other constructions}
  given a run $x$ of $\largesys$, we construct local runs $\yflood(A^1)$, $\yflood(B^1)$, $\yflood(B^2)$, \ldots, $\yflood(B^c)$ for the processes of the cutoff system. The construction ensures that
	\begin{enumerate}
	\item $\yflood(A^1)=x(A^1)$ and $\yflood(B^1)=x(B^1)$, and 
	\item when combined into a sequence of pseudo-configurations of $\cutoffsys$, the resulting sequence $\yflood$ is a pseudo-run that is not deadlocked, i.e., it evolves according to enabled transitions of the processes and at least one process moves infinitely often. 
	\end{enumerate}
	To ensure the latter, we devote to every state $q \in T_B$ that is reached in run $x$ one local run of template $B$ that moves into $q$ as fast as possible, and then stutters there forever.
  
  \item \emph{Interleaving Construction}:
The interleaving construction converts the pseudo-run $\yflood$ into the desired run $y$ by restoring an interleaving semantics. To this end, it may add local stuttering of one or several processes to ensure that at most one process moves at any time, and it may remove global stuttering to ensure that at least one process moves. The resulting run $y$ satisfies $y(A^1, B^1)\simeq x(A^1, B^1)$ and is not deadlocked.
\end{enumerate}

In the following, we formalize these two constructions. 

\subsubsection*{Flooding Construction.}
Set $\yflood(A^1)=x(A^1)$, $\yflood(B^1)=x(B^1)$.
Since $x$ satisfies the property, it must in particular be infinite, and hence there is a process of $\largesys$ that moves infinitely often in $x$.
If this process is a copy of $B$, say $B^\infty$, then set $\yflood(B^c) = x(B^\infty)$. Otherwise it is process $A^1$, and we set $\yflood(B^c)=\yflood(B^1)$.
To make sure that all local transitions in $\yflood(A^1)$, $\yflood(B^1)$ and $\yflood(B^c)$ are enabled, we construct additional local runs $\yflood(B^i)$ for $i\in [2,c-1]$ in the following way.

Let $\visited \subseteq T_B$ be the set of all local states of $B$ that are visited by at least one process in the run $x=(s_1,e_1,p_1) (s_2,e_2,p_2) \ldots$ of $\largesys$, i.e.:
$$\visited = \{ q \in T_B \| \exists{\time \in \bbN}\ \exists{i \in [1,n]}: s_\time(B^i) = q \}.$$

For $q \in \visited$ let:
\begin{itemize}
\item $\first_q = min(\{ \time \| \exists{i}: s_\time(B^i) = q\})$ be the first point in time where state $q$ is visited, and 

\item $\witfirst_q = any(\{ i \| s_{\first_q}(B^i)=q \})$ the index of a process that reached $q$ first (a ``witness'' process for $q$).

\end{itemize} 

Let $pr$ be an arbitrary bijection function from $\visited$ to $[2,|\visited|+1]$.
We use $pr$ to map a state $q \in \visited$ to a process $B^{pr(q)}$ of $\cutoffsys$.

For every $q \in \visited$, set
$$ \yflood(B^{pr(q)}) = \left(x(B^{\witfirst_q})\slice{1}{\first_q}\right)(q,e)^\omega,
$$
where $e$ is the local input of process $B^{pr(q)}$ at moment $\first_q$.
In words, to every state of $\visited$ we devote one process in $\cutoffsys$ that reaches it (on the shortest local path known from $x$) and then stays there.

For every $p \in [|\visited|+2,c-1]$ (this set is empty if $\visited=T_B$), set 
$$ \yflood(B^p) = \yflood(B^1),$$
i.e., all processes that do not `flood' states from $\visited$ repeat transitions of the process $B^1$.

\begin{figure}[h]
% \setlength{\abovecaptionskip}{-7pt plus 3pt minus 2pt} % Chosen fairly arbitrarily 
\centering
\scalebox{0.7}{
\input{img/disj_flooding_construction}
}
\caption{Illustration of the flooding construction from Lemma \ref{disj:le:NonFairDisjunctiveBounding}.\ak{Add flooding of the init state}}
\label{disj:fig:FloodingConstruction}
% \vspace{-5pt}
\end{figure}

Thus, we have defined all local runs $\yflood(A^1), \yflood(B^1), \yflood(B^2), \ldots$ in $\cutoffsys$. We obtain a sequence of pseudo-configurations $\yflood=(\sflood_1,\eflood_1,\Pflood_1)\ldots$ in the obvious way by defining the $\sflood_\time$ and $\eflood_\time$ as tuples of the corresponding local states, and letting the $\Pflood_\time$ contain all processes of $\cutoffsys$ that transit between state $\sflood_\time$ and $\sflood_{\time+1}$.\sj{$\leftarrow$ have this outside, in a definition?}
Any $\Pflood_\time$ may contain multiple processes that take a transition at the same time, e.g., if $\witfirst_q = i = \witfirst_{q'}$ for $q\neq q'$, then a prefix of $x(B^i)$ is contained in both $\yflood(B^{pr(q)})$ and in $\yflood(B^{pr(q')})$.
There might be also elements with $\Pflood_\time=\emptyset$. This happens if $p_\time \not\in \{ B^i \| \exists{q} \in \visited:\ i = \witfirst_q \} \cup \{B^1,B^\infty\}$, i.e., $p_i$ is a process that is not used to construct a local run of $\cutoffsys$. Figure~\ref{disj:fig:FloodingConstruction} illustrates the flooding construction.\ak{illustrate issues mentioned below?}

We show that the resulting sequence $\yflood = (\sflood_1,\eflood_1,\Pflood_1)\ldots$ is a pseudo-run of $\cutoffsys$. To this end, observe that the flooding construction ensures the following properties:
\begin{enumerate}
\item [P1.]
$\yflood(A^1,B^1) \simeq x(A^1,B^1).$

\item [P2.]
$\forall{q \in \visited}\ \forall{\time \ge \first_q}:\ \sflood_\time(B^{pr(q)}) = q.$

\item [P3.]
At any point of $\yflood$, if some process of $\cutoffsys$ transits $\transition{q}{q'}{e:g}$, then at the same point of the run $x$ of $\largesys$ there is a process that makes exactly the same transition $\transition{q}{q'}{e:g}$.
% $\forall{i} \ \forall{(p^*\!:\!\transition{q}{q'}{e:g})}:$
% $$(p^*\!:\!\transition{q}{q'}{e:g}) \in (s^*_i \rightarrow s^*_{i+1})
% ~~\impl~~
% \exists{p}\ (p\!:\!\transition{q}{q'}{e:g}) \in  (s_i \rightarrow s_{i+1}),$$
% where $p^*$ is a process of $\cutoffsys$ and $p$ is a process of $\largesys$.
\item [P4.]
At any point of $\yflood$, if more than one process transits, then they make exactly the same transition.
\end{enumerate}

We need to show that every element $(\sflood_{\time+1},\eflood_{\time+1},\Pflood_{\time+1})$ is derived from element $(\sflood_\time,\eflood_\time,\Pflood_\time)$ by local transitions of all processes in $\Pflood_\time$. 
Suppose that $p \in \Pflood_\time$, and the local transition from $q=\sflood_\time(p)$ to $q'=\sflood_{\time+1}(p)$ (with local input $\eflood_\time(p)$) is guarded by some guard $g \subseteq T_A \cup T_B$. Then by property P3 some process of $\largesys$ makes exactly the same transition, and hence in $s_\time$ of $x$ there is a process in some state $r \in g$. Consider two cases:
\begin{itemize}
  \item if $r \in T_A$, then by property P1, we have $\sflood_\time(A^1)=r$, and thus the transition is enabled.
  \item if $r \in T_B$, then $\time \ge \first_r$.
  Note that $p \neq B^{pr(r)}$ (since process $B^{pr(r)}$ does not move after reaching $r$ at time $\first_r$), and hence the transition is enabled.
\end{itemize}
 
\subsubsection*{Interleaving Construction.}
To obtain a run $y$ with $y(A^1, B^1)\simeq x(A^1, B^1)$ from $\yflood$, we first\rb{what is second?} sequentialize simultaneous transitions of processes.

Let $\interleave$ be the function that takes as input a pseudo-run $(\sflood_1,\eflood_1,\Pflood_1)$, $(\sflood_2,\eflood_2,\Pflood_2)$\ldots from the flooding construction and returns the pseudo-configuration sequence $\pi_1 \cdot \pi_2 \cdot \ldots$, where the $\pi_\time$ are non-empty sequences constructed from $(\sflood_\time, \eflood_\time, \Pflood_\time)$ in the following way:
\begin{itemize}
  \item if $|\Pflood_\time|\le 1$, then $\pi_\time = (\sflood_\time, \eflood_\time, \Pflood_\time)$,
 
  \item otherwise, $\Pflood_\time$ contains several processes that move simultaneously, say $p_1,\ldots,p_n$. By property P4, we know that in this case $p_\time \in \{ B^1,\ldots,B^c\}$ for all $\time$.
	%Then:
%  $\transition{s_\time(p_1)}{s_{\time+1}(p_1)}{e_\time(p_1)}$,
%  $\ldots$, 
%  $\transition{s_\time(p_n)}{s_{\time+1}(p_n)}{e_\time(p_n)}$.
  Then $\pi_\time = (s_{\time_1},e_{\time_1},P_{\time_1}) \ldots (s_{\time_n}, e_{\time_n}, P_{\time_n})$, where:
  \begin{itemize}
  \item 
  $(s_{\time_1}, e_{\time_1}, P_{\time_1}) = (\sflood_\time, \eflood_\time, \{ p_1 \})$, 
  \item 
  $s_{\time_2} = s_{\time_1}[s_{\time_1}(p_1) \gets \sflood_{\time+1}(p_1)]$, \\
  $e_{\time_2} = e_{\time_1}[e_{\time_1}(p_1) \gets \eflood_{\time+1}(p_1)]$, \\
  $P_{\time_2} = \{ {p_2} \}$;

  \item 
  \ldots
  \item 
  $s_{\time_n} = s_{\time_{n-1}}[s_{\time_{n-1}}(p_n) \gets \sflood_{\time+1}(p_n)]$, \\
  $e_{\time_n} = e_{\time_{n-1}}[e_{\time_{n-1}}(p_n) \gets \eflood_{\time+1}(p_n)]$, \\
  $P_{\time_n} = \{ {p_n} \}$.
  \end{itemize}
  Note that $\sflood_{\time+1} \equiv s_{\time_n}[s_{\time_n}(p_n) \gets \sflood_{\time+1}(p_n)]$.
\end{itemize}

It is straightforward to show that $\interleave(\yflood)$ is a pseudo-run of $\cutoffsys$ where at each moment either one or no process moves, and $y(A^1,B^1) \simeq x(A^1,B^1)$.
Thus, let $y = \destutter(\interleave(\yflood))$ to obtain the desired run\footnote{Note that $\destutter(x)$ is finite for a run $x$ that ends in an infinite repetition of the same configuration $(s,e,p)$. We abuse the notation and write $\destutter(x)$ for $\destutter(x)\ (s,e,p)^\omega$ in this case.}
of $\cutoffsys$.
This concludes the proof of $\implies$ direction.

\bigskip
\noindent Direction $\impliedby$\sj{if we keep Monotonicity Lemma, this is just repeated application}\ak{but then you need to prove Monotonicity Lemma?} (proof idea):\\
Construct the run $y$ of the large system $\largesys$ from a given run $x$ of the cutoff system $\cutoffsys$ as follows: $y(A^1)=x(A^1)$, $y(B^i)=x(B^i)$ for $i\in [1,c]$, and $y(B^{c+i}) = x(B^c)$ for $i \in [1,n-c]$. 
Use the interleaving construction to restore the interleaving semantics of the resulting pseudo-run to obtain $y$.
% 
\end{proof}

==> proof-idea-disj-bounding-fair.tex <==
\begin{proof}[Proof idea]
\noindent Direction $\implies$:
\sj{for weak or strong fairness, the same construction can be used; evacuation is not necessary, but also doesn't increase the cutoff if we use it; difficulty: show that cutoff is still tight
}
Let $c=2\card{B}$. Given an unconditionally-fair run $x$ of a system $\largesys$ we construct an unconditionally-fair run $y$ of the cutoff system $\cutoffsys$ such that $y(A,B_1)\simeq x(A,B_1)$.

The construction of $y$ can be separated into four parts, three of which are 
modifications of constructions seen in the previous lemmas:
\begin{enumerate}
  \item \emph{Flooding Construction}: We construct from $x$ a pseudo-run $
\yflood$ of $\cutoffsys$ with i) $\yflood(A,B_1) = x(A,B_1)$, ii) 
\emph{two} witness processes for every $q \in \visited_\inf(x)$, and iii) one witness 
process for every $q \in \visited_\fin(x)$.
	\item \emph{Evacuation Construction}: 
	Like in the proof of Lemma~\ref{le:disj:deadlocks}, we need to ensure that 
witness processes for states from $\visited_\fin(x)$ will leave their states. In 
this case, this is necessary because otherwise we cannot guarantee that they will 
be able to move infinitely often. Let $\yevac$ be the resulting pseudo-run, and let 
$\pref$ be the first moment such that in $\yevac[\pref:\infty]$ 
all processes except $A$ and $B_1$ are only in states from $\visited_\inf(x)$.
 
  \item \emph{Fair Extension}:
The fair extension turns the pseudo-run $\yevac$ into a unconditionally-fair pseudo-run $\yfair$.
The idea stems from the observation that in the original run $x$ of $\largesys$, all processes move infinitely often, and thus every local run must contain at least one loop.
To obtain a unconditionally-fair pseudo-run, we let all processes except $A$ and $B_1$ move along such loops after the moment $\pref$, while ensuring the property that there is always at least one process in every state from $\visited_\inf$.

  \item Interleaving Construction: takes the unconditionally-fair pseudo-run from the previous step and turns it into the desired unconditionally-fair run of $\cutoffsys$.
 
\end{enumerate}

\bigskip\noindent
Direction $\impliedby$: Repeated application of the Monotonicity Lemma.
\end{proof}


==> proof-idea-disj-bounding.tex <==
\begin{proof}[Proof idea]
We separate the proof into two main constructions that will be re-used in later proofs.
Let $c = \card{B}+2$ and $n \geq c$. In the following, we will call $\largesys$ the \emph{large system}, and $\cutoffsys$ the \emph{cutoff system}.

\medskip
\noindent
Direction $\implies$:\\
Let $x=(s_1,e_1,p_1), (s_2,e_2,p_2) \ldots$ be a run \sj{should runs start with $0$ or $1$?} of $\largesys$ that satisfies $\pexists h(A,B^{(1)})$.
We can construct a run $y$ of the cutoff system $\cutoffsys$ such that $y(A, B_1)\simeq x(A, B_1)$, using the following two steps: 
\begin{enumerate}
  \item \emph{Flooding Construction}:\sj{TODO: separate flooding from other constructions}
  given a run $x$ of $\largesys$, we construct local runs $\yflood(A)$, $\yflood(B_1)$, $\yflood(B_2)$, \ldots, $\yflood(B_c)$ for the processes of the cutoff system. We let $\yflood(A,B_1) = x(A,B_1)$, ensuring that the resulting run will satisfy the property $h(A,B^{(1)})$. To ensure that all transitions of $A$ and $B_1$ are enabled, we may need other processes that are in certain local states at a given time. Let $\visited(x) \subseteq T_B$ be the set of all $B$-states that are reached in run $x$. We devote to every $q \in \visited(x)$ one copy of template $B$ that moves to state $q$ on the shortest path exhibited in $x$, and then stutters there forever. Thus, at every point in time $t$ if there is a process $B_i$ with $x_t(B_i)=q$, then we also have a process $B_j$ with $\yflood_t(B_j)=q$. Finally, if neither $A$ nor $B_1$ move infinitely often in $x$, we need to add another copy of $B$ to $\yflood$, with some local run from $x$ that moves infinitely often. All transitions of this process will be enabled by the same argument as above for $A$ and $B_1$.

\begin{figure}[h]
% \setlength{\abovecaptionskip}{-7pt plus 3pt minus 2pt} % Chosen fairly arbitrarily 
\centering
\scalebox{0.7}{
\input{img/disj_flooding_construction}
}
\caption{Illustration of the flooding construction.\ak{Add flooding of the init state}}
\label{disj:fig:FloodingConstruction}
% \vspace{-5pt}
\end{figure}
  
  \item \emph{Interleaving Construction}:
	Note that in the resulting (pseudo-)run $\yflood$ we may have steps where multiple processes move at the same time, or where no process moves. The interleaving construction converts $\yflood$ into the desired run $y$ by restoring an interleaving semantics. To this end, it may add local stuttering of one or several processes to ensure that at most one process moves at any time, and it may remove global stuttering to ensure that at least one process moves. The resulting run $y$ satisfies $y(A, B_1) \simeq x(A, B_1)$ and is not deadlocked.
\end{enumerate}


Direction $\Longleftarrow$:
By repeated application of the Monotonicity Lemma.
\end{proof}

==> proof-idea-disj-deadlock-fair.tex <==
\begin{proof}[Proof idea]
% Note that if system $\largesys$ has a global deadlock, then the fairness does not influence the cutoff, and exactly the same proof as in Lemma~\ref{le:disj:deadlocks}, case `Global Deadlocks', can be reused here (with the cutoff being $|B|$). 
% For this reason, below we consider only the case of strictly local deadlocks.
 
\sj{Need high-level version of this.} Given a deadlocked and strong-fair if infinite run $x$ of $\largesys$, we construct a deadlocked and strong-fair if infinite run $y$ of $\cutoffsys$. The proof combines the ideas from all previous proofs, in particular flooding to enable all transitions, evacuation to ensure that deadlocked states will stay deadlocked \emph{and} that all others can move infinitely often, and fair extension for those processes that are not deadlocked.
%
%\begin{enumerate}
%\item 
%Define $\visited_\bot$ to be the set of locally deadlocked states in the run $x$. 
%Further, let $\visited_\bot^1$ be the set of locally deadlocked states that are only deadlocked if there is no other process in the same state, and $\visited_\bot^2 = \visited_\bot \setminus \visited_\bot^2$, i.e., the set of states that are locally deadlocked even if there was another process in the same state. 
%Denote the set of processes of $\largesys$ that are deadlocked in $\visited_\bot^2$ by $P_\bot^2$, and those in $\visited_\bot^1$ by $P_\bot^1$. 
%Note that $\card{P_\bot^1} = \card{\visited_\bot^1} \le \card{B}$, since by definition there can be at most one process in each state.
%
%\item Re-define $\visited_\fin$\sj{usually $\visited_\fin$ is defined in terms of $\visited_\inf$}, $\first_q$, $\last_q$, $\witfirst_q, \witlast_q$ not to account for processes in $P_\bot^1$, for example $\first_q = min(\{ i \| \exists{p \not\in P_\bot^1}: s_i(B^p) = q\})$.
%Re-define $\visited_\inf = \visited \setminus (\visited_\fin \cup \visited_\bot)$.
%Note that $\visited_\fin$ may have a non-empty interection with $\visited_\bot^1$, but $\visited_\fin \cap \visited_\bot^2 = \emptyset$\ak{only if the run is infinite!}\sj{we only have to consider infinite runs; for global deadlocks, proof is the same as without fairness; but how can $\visited_\fin \cap \visited_\bot$ be non-empty? deadlocked states will stay forever, and cannot be in $\visited_\fin$}.
%
%\item Set $\yflood(p)=x(p)$ for all $p \in \{A^1\} \cup P^1_\bot$. Also:
	%\begin{enumerate}
	%\item For each state in $\visited_\fin \cup \visited_\bot^2$ devote one flooding process in $\cutoffsys$.
%% 	Note that if in the run $x$ there is no process different from $P_\bot^1$ that visits state in $\visited_\bot^1$, then we do not flood this state.
	%\item For each state in $\visited_\inf$ devote two flooding processes in $\cutoffsys$.
	%\item For all processes of $\cutoffsys$ that are not used in the previous steps: if $\visited_\inf \neq \emptyset$ (the case of a strictly local deadlock), set their local run to be equal to the local run of one of $P_\inf$ processes, else if $\visited_\inf = \emptyset$ (the case of a global deadlock), then copy the behaviour of a process in $P_\bot^2$ (such process exists since $n > |B|$).
	%\end{enumerate}
%\item Evacuate processes in states $\visited_\fin$ by applying the standard evacuation construction.
%Note that the construction does not use local runs of processes from $P_\bot^1$ since we re-defined $\last$ and $\witlast$, and hence no process evacuates into state in $\visited_\bot^1$.
%
%\item After evacuation, all $B$ processes will be in $\visited_\inf \cup \visited_\bot^2 \cup \visited_\bot^1$.
%For those in $\visited_\inf$, apply the fair extension.
%\item Finally, we use $\destutter$ and $\interleave$ as usual\ak{cannot use destutter}\sj{destutter can also result in finite paths for non-deadlocked runs; but we can just mention that a finite path means that all processes only take self-loops}.
%\end{enumerate}
%
%The resulting configuration sequence is a run of $\cutoffsys$ by correctness of the flooding, evacuation, fair extension, interleaving and destuttering constructions\ak{we can say this only if use exactly the same flooding/etc. consructions before -- i.e., don't account for processes that we copy}. 
%Furthermore, for every $q \in \visited_\bot^1$ we have exactly one process in $\cutoffsys$ that eventually stays in $q$, and for every $q \in \visited_\bot^2$ -- at least one such process; they are eventually locally deadlocked in $q$ because the states that appear infinitely often in the run $x$ of $\cutoffsys$ are the same as in the resulting run of $\largesys$.
%
%How many processes does the construction use?
%The first answer would be $|\visited_\fin| + |\visited_\bot^2| + |\visited_\bot^1| + 2|\visited_\inf| \leq 2|B|$ 
%(since $|\visited_\fin| + |\visited_\bot^1| \leq 2|\visited_\fin \cup \visited_\bot^1|$, and the sets $\visited_\bot^1 \cup \visited_\fin$, $\visited_\bot^2$, $\visited_\inf$ are disjoint).
%But we can reduce it to $2|B|-1$ (and later prove that it is tight) if analyze the cases\ak{this is crazy and should be double-checked\ldots}\sj{gist: at least one state of $B$ is in $\visited_\fin$ and is evacuated either to $\visited_\inf$ (in which case we drop one of the two other copies for that state), or into $\visited_\bot^2$ (in which case we have $3$ copies for these two states)}: 
%\begin{enumerate}
%\item 
%Process $A^1$ deadlocks. 
%Two cases are possible: $A^1$ deadlocks in a terminal state\ak{does terminal state contain transitions guarded with states of $A$?}\sj{terminal state is not defined} -- then use the standard flooding construction until $A^1$ reaches the terminal state, and then schedule processes arbitrarily strong-fair if possible. 
%This gives the cutoff $|B|$.
%
%The second case -- $A^1$ deadlocks in a non-terminal state guarded with a state $r$ of $B$ process.
%Let $uniq = \visited_\fin \oplus \visited_\bot^1$ (symmetric difference), then 
%\begin{align*}
%& |\visited_\fin| + |\visited_\bot^2| + |\visited_\bot^1| + 2|\visited_\inf| = \\
%& 2(|\visited_\fin \cap \visited_\bot^1| + |uniq| + |\visited_\bot^2| + |\visited_\inf|) - \\
%&~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ - |\visited_\bot^2| - |uniq|.
%\end{align*}
%Now note that $r \not\in \visited_\inf \cup \visited_\bot^1 \cup \visited_\bot^2$, and consider two cases: 
%i) $r \in uniq$: $|uniq|>0$ and hence the result is $\leq 2|B|-1$; 
%ii) $r \not\in uniq$: hence the result is $\leq 2|B|-2$.
%Hence, the cutoff $2|B|-1$.
%
%\item 
%Process $A^1$ moves infinitely often, and hence there is at least one $B$ process that deadlocks.
%Similarly to the previous case: if the $B$ process deadlocks in the terminal state, then $c=|B|+1$\ak{or $|B|$?}.
%Consider two cases: 
%\begin{enumerate}
%\item 
%$B$ deadlocks in state $q$ and $q \in \visited_\bot^2$.
%Hence, $|\visited_\bot^2|>1$ and the equation results in $\leq 2|B|-1$.
%
%\item 
%$B$ deadlocks in state $q$ and $q \in \visited_\bot^1$.
%If $q \in uniq$, then the equation results in $\leq 2|B|-1$.
%If $q \not\in uniq$, then $q \in \visited_\fin \cap \visited_\bot^1$.
%In this case observe that the process that visited state $q$ and then exited it in the run $x$, entered some state not in $\visited_\bot^1$ (by definition of $\visited_\fin$).
%If the process entered state in $\visited_\bot^2$, then $|\visited_\bot^2|>1$ and the equation results in $\leq 2|B|-1$.
%If the process entered state $q' \in \visited_\inf$, then modify the construction: instead of devoting two processes that flood state $q'$, devote only one process.
%This results in the cutoff $\leq 2|B|-1$.
%\end{enumerate}
%\end{enumerate}
%This concludes the proof.
\end{proof}
%----

==> proof-idea-disj-deadlock.tex <==
\begin{proof}[Proof idea]
\ak{status -- possibly unite/shorten parts of the proofs}
We prove that if there is a deadlocked run $x$ of the large system $\largesys$, then there also is a deadlocked run of the cutoff system $\cutoffsys$ ($c$ is defined later)\rb{c is $B+1$? otherwise introduce $c_1$ and $c_2$ -- cutoffs for two different cases}. 
To this end, distinguish two cases: either $x$ is strictly locally deadlocked (and thus infinite), or it is globally deadlocked (and thus finite).

\subsubsection*{Strictly Locally Deadlocked Run.}
Again, we can distinguish two cases: 
\begin{itemize}
\item [a)] process $A$ deadlocks, hence wlog. process $B_1$ moves infinitely often,
\item [b)] process $A$ moves infinitely often, hence wlog. process $B_1$ deadlocks.
\end{itemize}
Then we construct an infinite run $y$ of the cutoff system $\cutoffsys$ such that process $U \in \{A,B_1\}$ is deadlocked in $y$ iff it is deadlocked in $x$. In the following, let $U$ be the process that eventually deadlocks, and $V$ the process that moves infinitely often.

Let $c=|B|+1$.

Recall that process $U$ is locally deadlocked in $x=(s_1,e_1,p_1) \ldots$ iff there is a $\time$ such that all transitions of $U$ from $s_{\time'}(U)$ with $e_{\time'}(U)$ are disabled in all states $s_{\time'}$ with $\time' \geq \time$. Note that by definition, if $U$ does not move then $s_{\time'}(U) = s_\time(U)$ and $e_{\time'}(U)=e_\time(U)$ for $\time' \geq \time$.

Informally, the construction consists of the following three steps:
\begin{enumerate}
\item \emph{Flooding Construction.} To ensure that processes $U$ and $V$ 
can exhibit the same behavior as in $x$ until the moment where one of them 
deadlocks, we first use the flooding construction from the proof of 
Lemma~\ref{disj:le:NonFairDisjunctiveBounding}, except that we do not need an 
additional process that moves infinitely often.\sj{here it is important 
that flooding construction only considers processes different from $B^1$ --- 
but this should be OK in other cases also?}\ak{todo: flooding here is applied to the whole run, not to local runs as i imagined before}

\item \emph{Evacuation Construction.} The evacuation construction modifies some of the local runs that result from the flooding construction. Since the local deadlock of $U$ may 
depend on the fact that eventually some states $q \in \visited(x)$ will not be 
visited anymore, we distinguish between states that are visited finitely often 
($\visited_\fin(x)$) or infinitely often $(\visited_\inf(x))$ in $x$. For states 
$q \in \visited_\fin(x)$, we require that their witness processes leave $q$ 
eventually and move to some state from $\visited_\inf(x)$. This is always 
possible by mimicking the behavior of the last process that left $q$ in the 
original run $x$, retaining the order in which states are moved out of 
$\visited_\fin(x)$ in the original run $x$.

If all processes are eventually in states from $\visited_\inf$, then 
$U$ is also deadlocked in the constructed run: if it was not, then one of the 
states from $\visited_\inf$ would enable one of its transitions, and 
therefore $U$ would not be deadlocked in $x$. Thus, we obtain a pseudo-run 
in which $U$ deadlocks.

\item \emph{Interleaving Construction.} Like in the proof of Lemma~\ref{disj:le:NonFairDisjunctiveBounding}, we use the interleaving construction to convert the resulting pseudo-run into a run.
\end{enumerate}

\subsubsection*{Globally Deadlocked Run $x$.}
In a similar way, we can construct a globally deadlocked run $y$ of $\cutoffsys$ with $c = 2 \card{B} - 1$ from a globally deadlocked run of $\largesys$. The additional copies are needed since we have to copy all local runs that end in a state $q$ that is only deadlocked if there is not other process in $q$ (bounded by $\card{B}$), and in addition use the flooding and evacuation construction for all states that are visited in the other local runs of $x$ (bounded by $\card{B}$). A closer investigation of the possible cases gives a cutoff of XXX.
\end{proof} 

==> proof_defs.tex <==
\noindent\hrulefill

For a given infinite path $x$ of $\largesys$ we distinguish between states of template $B$ that are visited finitely and infinitely often along $x$: 
\begin{itemize}
\item
$\visited = \{ q \in T_B \| \exists{j \in \bbN}\ \exists{p \in [1,n]}: s_j(B^p) = q \}$,
\sj{for deadlocks, these should only be the states visited by $p \in [2,n]$ --- is this OK in all cases?}

\item 
$\visited_\inf = \{ q\in T_B \| \forall{i} \in \bbN \ \exists{j>i}\ \exists{p \in [1,n]}: s_j(B^p)=q \}$,
 
\item 
$\visited_\fin = \visited \setminus \visited_\inf$.
\end{itemize}
%
Let $\last_\fin$ be the last point in run $x$ with a process in a state from $\visited_\fin$, i.e.: 
$$\last_\fin = max(\{ i \in \bbN \| \exists{p \in [1,n]}: s_i(B^p) \in \visited_\fin \}).$$
Let $\first_\inf$ be the first point in run $x$ where all states from $\visited_\inf$ have been visited at least once, i.e.:
$$\first_\inf = min(\{ i \in \bbN \| \forall{q\in \visited_\inf}\ \exists{j\le i}\ \exists{p \in [1,n]}: s_j(B^p)=q \}).$$
%
Since run $x$ is infinite, process $B^1$ visits some state $q \in \visited_\inf$ infinitely often. 
Denote this state by $\qstar$, and denote the moment when $B^1$ reached $\qstar$ for the first time after $max(\last_\fin+1,\first_\inf)$\footnote{Intuitively, $max(\last_\fin+1, \first_\inf)$ is the first moment in $x$ when $B$-processes exited $\visited_\fin$ and visited all states in $\visited_\inf$ at least once.} by $\pref$, i.e.:
\begin{align*}
& \qstar = any(\{ q \in T_B \| \forall{i \in \bbN} \ \exists{j \ge i}: s_j(B^1) = q\}), \\ 
% & \estar= any(\{ e \| \forall{i} \ \exists{j \ge i}: (s_j(B^1),e_j(B^1)=(\qstar,e) \}), \\ 
& \pref = min( \{ i \ge max(\last_\fin+1,\first_\inf) \| s_i(B^1)=\qstar \}).
\end{align*}\rb{isn't it $any(..) = any(visited_{inf})$ here?}

Intuitively, $\pref$ is the first moment of run $x$ when: all states in $\visited_\inf$ were visited, no process is in a state from $\visited_\fin$, and process $B^1$ is in the state $\qstar$ (which it visits infinitely often in $x$).
Note that all transitions in $x$ that happen after point $\pref$ must be enabled by some state in $\visited_\inf$, since only these states appear after $\pref$. Thus, if in the cutoff system there is at least one process (other than the one making the transition) in every state of $\visited_\inf$, then every transition that happened in $x$ after $\pref$ will be enabled.

For $q \in \visited$ let:
\begin{itemize}
\item $\first_q = min(\{ i \| \exists{p}: s_i(B^p) = q\})$ --- the first moment when state $q$ is reached, 

\item $\witfirst_q = any(\{ p \| s_{\f_q}(B^p)=q \})$ --- the index of a process that reached $q$ first,

\item 
$\last_q = max(\{ i \| \exists{p}: s_i(B^p) = q\})$ if $q\in \visited_\fin$ otherwise $\last_q = \pref$ --- the last point in $x[1:\pref]$ where state $q$ was seen,
 
\item $\witlast_q = any(\{ p \| s_{l_q}(B^p)=q \})$ --- the index of a process that was in $q$ last.
\end{itemize} 
Note that for any $q\in \visited_\fin$  $\first_q$ and $\last_q$ are in $[1,\last_\fin]$, and for any $q \in \visited_\inf$ $\first_q \in [1,\first_\inf]$, $\last_q \in [1,\pref]$.

% Finally, define $\ppi{q}$ and $\ei{q}$: for any state $q \in \visited_\inf$, there is a process of $\largesys$ and a local input $\ei{q}$ that appear infinitely often in $x=(s_1,e_1,sch_1)\ldots$\footnote{The existence of $\ei{q}$ follows from the fact that process inputs are finite while the run $x$ is infinite -- the construction can be adapted for inputs from infinite domains.}.
% Denote such process input by $\ei{q}$ and such process by $\ppi{q}$, i.e.:
% $$\ppi{q} = any(\{ B^p \| \forall{i}\ \exists{j\ge i}: s_j(B^p) = q \ \land \ e_j(B^p)=\ei{q}\}).$$


\noindent\hrulefill

==> tight-conj-prop-fair.tex <==
% 
\begin{proof} 
Exactly the same example (Fig.~\ref{fig:conj:tight_dead_tmpl}) as in Observation~\ref{obs:conj:tight_deadlock} can be used to prove the observation.
Note that if change the template $A$ to any that never deadlocks, then we get the example to prove the tightness for the special case of strictly local deadlocks too.
% \begin{figure}[Htb]
% \centering
% \subfloat[Template A]{
% \centering
% \makebox[0.4\textwidth][c]{
% \scalebox{0.75}{\input{img/conj_tight_deadlock_tmplA}}
% \label{fig:conj:tight_deadlock_tmplA}
% }}
% \subfloat[Template B]{
% \centering
% \makebox[0.6\textwidth][c]{
% \scalebox{0.75}{\input{img/conj_tight_deadlock_tmplB}}
% \label{fig:conj:tight_deadlock_tmplB}
% }}
% \caption{Templates $(A,B)$ used to prove the tightness of the cutoff $c=2|B|-2$ for the deadlock detection in 1-guard conjunctive systems.
% In the figure the edge with $\forall{\neg b_1},\ldots,\forall{\neg b_k}$ denotes edges with guards $\forall{\neg b_1},\ldots,\forall{\neg b_k}$ (Observation~\ref{obs:conj:tight_deadlock}).\ak{check me}}
% \label{fig:conj:tight_dead_tmpl}
% \end{figure}
\end{proof}
